Technical Report: Optimizing Human Involvement for Entity Matching and Consolidation

An end-to-end data integration system requires human feedback in several phases, including collecting training data for entity matching, debugging the resulting clusters, confirming transformations applied on these clusters for data standardization, and finally, reducing each cluster to a single, canonical representation (or "golden record"). The traditional wisdom is to sequentially apply the human feedback, obtained by asking specific questions, within some budget in each phase. However, these questions are highly correlated; the answer to one can influence the outcome of any of the phases of the pipeline. Hence, interleaving them has the potential to offer significant benefits. In this paper, we propose a human-in-the-loop framework that interleaves different types of questions to optimize human involvement. We propose benefit models to measure the quality improvement from asking a question, and cost models to measure the human time it takes to answer a question. We develop a question scheduling framework that judiciously selects questions to maximize the accuracy of the final golden records. Experimental results on three real-world datasets show that our holistic method significantly improves the quality of golden records from 70% to 90%, compared with the state-of-the-art approaches.

==> src/others.tex <==
%!TEX root = main.tex


%asks human to check whether the value $v$ should be repaired to another value $v'$ for all records containing value $v$. We repair the data using the GR questions that are approved by the human. 


%To improve the quality of marjory voting, Next we run GR (golden record) and get a set $Q_{GR}$ of GR questions, where 


%we can use active learning to get more matching/un-matching  pairs and feed them to entity matching to improve the matching quality. We require to ask the human to validate the pairs. 

%We generate a golden record as follows. 
%Based on the set of matching pairs $P$, it groups the entities into clusters such that two records $r_1,r_2$ in the same cluster if and only if $(r_1,r_2)\in P$. Based on matching pairs $P$, it can get a set $C$ of clusters.
%to get a set of clusters by providing some training data (e.g., matching/non-matching pairs by asking a set $Q_{EM}$ of EM questions).



\subsection{Data Integration Components}

%\subsubsection{Data Integration}

Let $\{D_1, \ldots, D_m\}$ be a set of relational tables from disparate data sources.
%
Let $R_i$ ($i\in [1,m]$) be the relational schema of $D_i$. 
%
Let $R$ be the schema that aligns attributes across all schemas $\{R_1, \ldots, R_m\}$, where $R \subseteq R_i$ ($i \in [1, m]$).
%
Informally speaking, {\em data integration} is to combine these $m$ tables into a unified view $D$ that is an instance of scheme $R$.
%
Traditionally, data integration typically consists of the following four consecutive processes:

\be
	\itemsep-1mm\parsep-1mm
	\item {\em Data Preparation:} normalize and clean each table $D_i$.
	\item {\em Scheme Integration (SI):} find the aligned scheme $R$.
	\item {\em Entity Matching (EM):} union $\{D_1, \ldots, D_m\}$ based on $R$, and produce clusters  (\ie groups of duplicates).
	\item {\em Entity Consolidation (EC):} compute for each cluster a golden record, which produces a set of golden records.
\ee

Note that in EM, we only consider the aligned attributes (\ie those attributes in $R$), while dropping the other attributes $\bigcup_{i\in[1,m]}R_i \setminus R$. That is, we do not consider ``data enrichment'' in this work, which also includes the attributes that belong to $R_i$ but not $R$ in the unified view $D$.

%\lgl{I will define the data later.}
%Let $R[\at{A_1},\at{A_2},\ldots,\at{A_n}]$ be a relation with $n$ attributes. Let $D$ be an instance (\ie a table) of $R$. In practice, the tuples in $D$ may come from multiple data sources. After running off-the-shelf schema integration tools to align their schemas, they will be treated as one relation.

\subsubsection{Data Preparation}

We mainly consider data repairing operations for data preparation in this work, excluding other tasks such as information extraction.

Informally speaking, data repairing (DR) refers to {\em value update techniques} that change detected erroneous data values to possibly correct values.

We consider two types of repairing techniques:
{\em probabilistic} and {\em deterministic}.

%\lgl{we just say deterministic repairs here? and move the probabilistic repairs to related works?}

\stitle{Probabilistic repairs.} 
This refers to the type of techniques that there exist error detection tools that can tell {\em what is wrong}, but these tools cannot tell us how to change the detected errors, such as functional dependencies (FDs)~\cite{AbiteboulHV95}, conditional functional dependencies (CFDs)~\cite{DBLP:journals/tods/FanGJK08}, denial constraints (DCs)~\cite{DBLP:journals/pvldb/ChuIP13}.
%
Consequently, algorithms have been devised to infer the most likely correct repairs in a probabilistic way, such as holistic data cleaning~\cite{DBLP:conf/icde/ChuIP13}, HoloClean~\cite{DBLP:journals/pvldb/RekatsinasCIR17}, SAT-solvers based used in NADEEF~\cite{DBLP:conf/sigmod/DallachiesaEEEIOT13}.

\stitle{Deterministic repairs.} 
Different from probabilistic repairs, deterministic repairs can uniquely determine how to repair the data, such as fixing rules~\cite{DBLP:conf/sigmod/WangT14}, SQL UPDATE queries~\cite{DBLP:conf/sigmod/HeVSLMPT16}, and string transformation programs~\cite{DBLP:journals/pvldb/Singh16}.
One major benefit of deterministic repairs is that they are typically declarative, thus is interpretable to the users.

\stitle{Probabilistic vs. deterministic repairs.} 
Probabilistic repairs usually achieve higher recall, and deterministic repairs outperform in better precision, since the former is more aggressive and the latter is more conservative.
%
Arguably, deterministic repairs are more widely used in practice such as ETL rules, data wrangling in Trifacta~\cite{DBLP:conf/cidr/HeerHK15}.
%
Probabilistic repairs, on the other hand, may cause dangerous cascading effect, if they make some wrong repairs.

%Given a dataset $S$ (one or multiple tables) as input, the machine operations in data preparation can be formalized as follows:
%
%
%\bi
%	\itemsep-1mm\parsep-1mm
%	\item {\em Error detection (ED).}
%An error detection tool returns a set ${\bf E} =\{e_1, \ldots, e_k\}$ of errors, where each $e_i$ ($i \in [1, k]$) could be either a cell, a tuple, or a set of cells from different tuples (and possibly from different sources).
%	\item {\em Data repairing (DR).}
%A data repairing tool returns a set ${\bf U} =\{u_1, \ldots, u_l\}$ of repairs, where each $u_i$ ($i \in [1, l]$) is a value update $cell~c: v \la v'$ that updates the value of cell $c$ from $v$ to $v'$, where $v \neq v'$.
%\ei

{%\small
\mybox{
{\bf Discussion:} We can define a unified declarative language for data repairing, in order to interact with the user:
(1) SQL like languages; or
(2) If-then-else that can contain arbitrary declarative functions (\eg transformation programs or similarity functions).
Note that, Excel or Trifacta never runs heuristic repairs, and the reason is evident.
}
} % end of font

\subsubsection{Entity Matching}

The problem of {\em entity matching} is, given a unified table $D$ (the records in $D$ may come from different sources), to find a set of clusters ${\bf C} = \{C_1, \ldots, C_n\}$ where each cluster $C_i$ contains a set of tuples in $D$ pertaining to the same real-world object (\ie duplicates). Moreover, these clusters form a partition of $D$, \ie
$D = \bigcup_{i=1}^n C_i$, and $C_i \cap C_j = \emptyset$ if $i\neq j$.

Broadly speaking, there are machine learning (ML) based EM tools, such as Tamr~\cite{DBLP:conf/cidr/StonebrakerBIBCZPX13} and Magellan~\cite{DBLP:journals/pvldb/KondaDCDABLPZNP16}, and declarative EM rules such as disjunctive normal forms (DNFs)~\cite{DBLP:journals/pvldb/WangLYF11} and General Boolean Formulas (GBFs)~\cite{synthesizer}.


\subsubsection{Entity Consolidation}

The problem of {\em entity consolidation} is, given a cluster $C$, to find a unique representation of each attribute $\at{A_i}$, which consists of two cases:
\be
%\itemsep-1mm\parsep-1mm
	\item[(i)] {\em A canonical value:} 
	The values on the specific attributes are equivalent, syntactically or semantically.

	A typical solution is to learn a function $f(\cdot)$ (\eg a transformation program), such that given two values $x, y$ from the same domain, $f(x, y)$ will output a value $z$ that is the canonical value of both $x$ and $y$. Note that we do not enforce the conditions $z = x$ or $z = y$.
	
	\item[(ii)] {\em A preferred value:} 
	The values are not the same, but the user may have a preference. For example, if there are two records about Nan, $r_1$: {\em (Nan, 2010, Edinburgh)} and $r_2$: {\em (Nan, 2015, Qatar)}, the user may prefer the most current value drawn from $r_2$.
	
	We cannot learn a function in this case. Traditional methods~\cite{DBLP:conf/icde/FanGTY13} use partial orders across attributes to infer the preferred value. Consider the above example, the rule is ``{\em pick the affiliation that is the most recent}'': 
$t_1 \prec_{\at{year}} t_2 \ra t_1 \prec_{\at{affiliation}} t_2$.
\ee

Moreover, if there are unsolved conflicts within a cluster of values, we use the majority consensus (MC) to select the golden value.

As a result, EC will produce a set of golden values, ${\bf G} = \{g_1, \ldots, g_n\}$, where $g_i$ is the golden record of cluster $C_i$.

%\subsection{Machine Algorithms}
%
%Now we will define the input and output of machine algorithms.
%
%\subsubsection{Data Preparation}
%
%\stitle{Error detection.}
%Given a dataset $S$ (one or multiple tables) as input, an error detection tool returns a set ${\bf E} =\{e_1, \ldots, e_k\}$ of errors, where each $e_i$ ($i \in [1, k]$) could be either a cell, a tuple, or a set of cells from different tuples (and possibly from different sources).
%
%\stitle{Data repairing.}
%Given a dataset $S$ (one or multiple tables) as input, a data repairing tool returns a set ${\bf U} =\{u_1, \ldots, u_l\}$ of repairs, where each $u_i$ ($i \in [1, l]$) is a value update $cell~c: v \la v'$ that updates the value of cell $c$ from $v$ to $v'$ where $v \neq v'$.

%\stitle{Single Data Repairing.} The input includes a table $T$ and a repairing example $c\rightarrow c'$, and the output is a set of generalized repairings $\{o\rightarrow o'\}$. (The set can be clustered as several disjoint groups and the reparinings in each group are all true or false.)
%
%\stitle{Group Data Repairing.} The input includes a group of records, and a group repairing example $G \rightarrow G'$, and the output is a set of generalized repairings $\{o\rightarrow o'\}$. 

%\stitle{Entity Matching.} The input includes a table $T$ and a set of positive examples $P=\{r=r'\}$ and a set of negative examples $N=\{r\neq r'\}$, and the output is a set of disjoint groups where each group contains multiple records that potentailly refer to the same entity.


%\stitle{Entity Consolidation.} The input is a group of records (which is the output of entity matching) and the output is a golden record generated from the group. 



\subsection{Abstraction of Machine Operations}
\label{ssec:atools}

In this section, we will abstract the inputs and outputs of machine operations, for data repairing (DR), entity matching (EM), and entity consolidation (EC).

%We take existing tools on data repairing (DR), entity matching (EM), and entity consolidation (EC) as black-boxes. We next abstract their inputs and outputs.

%\stitle{$ED(T,E)\rightarrow E'$.} It takes a table $T$ and a set of given errors $E$ as input, where $E$ can be empty, and outputs a set of new detected errors.

%\lgl{we can remove error detection? only discuss data repairing? error detection can be taken as a sub-routine of data reparing? DR will generate a set of candidate repairs that need to ask human to check? if yes, we need to add a function for this.}

\subsubsection*{Data Repairing: \repair$(D, \QR)\rightarrow D'$} 

\bi
\itemsep-1mm\parsep-1mm
	\item {\bf Input:}
	\bi
	\itemsep-1mm\parsep-1mm
		\item $D$: a dataset (one or more tables).
		\item $\QR$: a set of pairs $\{(V, S)\}$, which represents the known errors and repairs.
		\bi
%		\itemsep-1mm\parsep-1mm
			\item $V$: a set of cells (to represent one cell, a tuple with multiple cells, and cells from multiple tuples that may come from different tables).
			\item $S \in \{\checkmark, \times, c\}$, where ``$\checkmark$'' means that $V$ is correct, ``$\times$'' indicates that $S$ is wrong, and $c$ is constant (\ie a data repair that the user confirms) to update $S$. %($S$ must be a single cell in this case). 
		\ei
	\ei
	\item {\bf Output:}	
	\bi
	\itemsep-1mm\parsep-1mm
		\item $D'$: a repaired dataset \wrt $D$ by value updates.
	\ei	
\ei

%\stitle{\repair$(D, \QR)\rightarrow D'$.} 
%It takes a dataset $D$ and a set $\QR$ as input, and outputs a repaired table $D'$. Here, $\QR$ is a set of pairs $\{(V, S)\}$, where $V$ is a set of cells (to represent only one cell, a tuple with multiple cells, and cells from multiple tuples), and $S \in \{\checkmark, \times, c\}$, where ``$\checkmark$'' means that $V$ is correct, ``$\times$'' indicates that $S$ is wrong, and $c$ is constant (\ie a data repair that a user provides) to update $S$ ($S$ must be a single cell in this case). 
%\lgl{what is a constant?} %nan: a constant is just a value that the user used to repair an error
%

Note that $\QR$ could be empty, indicating a cold start that is bootstrapped with no known errors/repairs.

%\lgl{do we need to remove fig 1? }
%\lgl{We use $Q_M, Q_C, Q_R$ instead of $\QM, \QC,\QC$. We need to make consistent.}

\subsubsection*{Entity Matching: $\ematch(D, \QM)\rightarrow {\bf C}$} 

\bi
\itemsep-1mm\parsep-1mm
	\item {\bf Input:}
	\bi
	\itemsep-1mm\parsep-1mm
		\item $D$: one or multiple tables with an aligned schema.
		\item $\QR$: a set of pairs $\{P, M\}$:
		\bi
%		\itemsep-1mm\parsep-1mm
			\item $P$: a pair of tuples $(r, s)$.
			\item $M \in \{\checkmark, \times\}$, where 
``$\checkmark$''/``$\times$'' are labels indicating that $r$ and $s$ are/aren't duplicates.

		\ei
	\ei
	\item {\bf Output:}	
	\bi
	\itemsep-1mm\parsep-1mm
		\item ${\bf C}$: a set of clusters.
	\ei	
\ei

Similarly, $\QM$ could be empty.

%\stitle{$\ematch(D, \QM)\rightarrow {\bf C}$.} 
%It takes a dataset $D$ and a set $\QM$ as input, and outputs clusters ${\bf C}$.
%Here, $\QM$ is a set of pairs $\{P, M\}$, where $P$ is a pair of tuples $(r, s)$ and $M \in \{\checkmark, \times\}$, where `$\checkmark$''/``$\times$'' means that $r$ and $s$ are/aren't duplicates.
%Similarly, $\QM$ could be empty.
%a set of positive matching pairs $M$ and a set of negative pairs $N$ as input, where $M,N$ can be empty, and outputs a set of groups, where each group contains multiple tuples that are taken as matching pairs.

\subsubsection*{Entity Consolidation: $\cons({\bf C}, \QC)\rightarrow {\bf G}$} 

\bi
\itemsep-1mm\parsep-1mm
	\item {\bf Input:}
	\bi
	\itemsep-1mm\parsep-1mm
		\item ${\bf C}$: a set of clusters.
		\item $\QC$: a set of  pairs $(C, g)$, where $g$ is the user selected value for the cluster $C \in {\bf C}$, which can be empty.
	\ei
	\item {\bf Output:}	
	\bi
	\itemsep-1mm\parsep-1mm
		\item  {\bf G}: all golden records for each cluster $C_i$ in ${\bf C}$.
	\ei	
\ei

%\stitle{$\cons({\bf C}, \QC)\rightarrow {\bf G}$.} 
%It takes clusters ${\bf C}$ and a set $\QC$ as input, and outputs {\bf G}, all golden records for each cluster $C_i$ in ${\bf C}$.
%
%Here, $\QC$ is a set of value update $\{cell: v\ra v'\}$, which can also be empty.

\subsection{Abstraction of Human Operations}
\label{ssec:human}

In the four data integration processes, schema integration is relatively easy, which can either be automatically performed by off-the-shelf tools, or by the users manually.
%
In other words, the main human time was spent on DP, EM and EC.
%
Below we discuss the common human operations (or questions) in different processes.

\subsubsection*{Data repairing}

We consider the following questions.

\be 
	\itemsep-1mm\parsep-1mm
	\item Is a cell wrong?
	\item Is a tuple wrong?
	\item Is a (small) set of values wrong? (For a violation.)
	\item Is the repair for a cell value from $v$ to $v'$ correct?
	\item Is the repair for a small set of values correct? %We can extend (4) to a small set of values.
	\item Is an integrity constraint or a declarative rule correct? 
	%\lgl{do we need it? which integrity constraint?} In falcon, we ask the user about an SQL update query, which belong to this category. If we don't have this category, who can validate the inferred or generalized rules?
\ee		

The answers from the above questions will be further used to infer/confirm integrity constraints, transformation programs, or declarative data cleaning rules.

\subsubsection*{Entity Matching}

Given a pair of tuples $(r, s)$, the user can answer:

\be 
	\itemsep-1mm\parsep-1mm
	\item Yes: they match; 
	\item No: they do not match; or
	\item Unknown. 
\ee

\subsubsection*{Entity Consolidation}

Given a set of values $V$ in the same column of the cluster, the user can:

\be 
	\itemsep-1mm\parsep-1mm
	\item Pick one value $v$ in $V$ as the golden value; or
	\item Unknown.
\ee	

\subsubsection*{Human Operations: \human$(I) \ra O$}

Below we abstract the input/output of human operations.

\bi
\itemsep-1mm
	\item {\bf Input:}
	\bi
	\itemsep-1mm
		\item $I$ (\ie a question to the user): one item in $\{cells, updates, queries\}$ and a description
		\bi
			\item {\em cell}s can represent either one cell, one tuple, two tuples, or multiple tuples;
			\item {\em updates} can represent one to many value repairs; 
			\item {\em queries} are for the declarative data repairing language, if we have;
			\item {\em description} is simply to explain the task such as ``is this an error" or ``are these two tuples duplicates"?
		\ei
	\ei
	\item {\bf Output:}	
	\bi
	\itemsep-1mm
		\item  {\bf O} (\ie an answer of a user feedback): in $\{\checkmark, \times, c\}$
	\ei	
\ei

%\stab
%\human$(I) \ra O$.
%The input $I$ is in $\{cells, updates, queries\}$ and a description; and the output $O$ is in $\{\checkmark, \times, c\}$.
%For input:
%cells can represent either one cell, one tuple, two tuples, or multiple tuples;
%updates can represent one to many value repairs; 
%queries are for the declarative data repairing language, if we have;
%and a description is simply to explain the task such as ``is this an error" or ``are these two tuples duplicates"?
%For output: $c$ is a constant, for one value repair.

These should be enough to capture all the questions discussed for data repairing, entity matching, and entity consolidation. 
Moreover, the answers (or the outputs) compile with the input (\ie $\QR$, $\QM$ and $\QC$ defined in Section~\ref{ssec:atools}) of existing tools.

%\lgl{do we need to use $c$? or just yes/no question?}

%\lgl{We need to abstract the human operation.}

%\stitle{Error Detection?} Do we need to use human to detector errors? how to?
%it is not clear how to define the human operations for error detection. which operation can suggest repairings?  
% Nan: error detection is included in data repairing already

\subsection{Online Data Integration}

We consider a set of data repairing (including error detection) tools, one entity matching tool, and one entity consolidation tool. These tools are either fully automatic (or unsupervised), or need to interact with users by asking questions (see Section~\ref{ssec:human}) and consume the user feedback.

\stitle{Problem statement.}
The problem of {\bf online data integration} is -- given a unified view $D$ from multiple data sources $\{D_1, \ldots, D_m\}$, a set of DR tools ${\cal U}$, one EM tool ${\cal M}$, one EC tool ${\cal C}$, and a budget $B$ for the number of questions a user can answer (we assume that each question takes a unit cost) as input -- to compute a consolidated set of (golden) records for all clusters while maximizing the accuracy (\ie precision and recall) of ${\bf G}$.

We denote the ground truth by ${\bf G}_{\at{gold}}$, which contains all golden records of the perfect clusters of duplicates.

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=\columnwidth]{overview.pdf}
\vspace{-2em}
\caption{Architecture}
\label{fig:arch}
\end{center}
\vspace{-1em}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Related Work}


%\subsection{System Framework}

%An overview of our ``online data integration'' system is shown in Figure~\ref{fig:arch}.

















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DR, EM, EC generates a set of questions $Q_R$, $Q_P$, $Q_C$. The question scheduler selects a question to ask. (We will discuss how to select $k$ questions to ask in parallel.) Based on the question and the answer, we rerun the tools. 


%Given the dataset $D$ a set of clusters $C'$ from the EC tool, a DR tool repairs $D$ and outputs a repaired data $D'$.

 \iffalse

The redlines in the figure show the workflow of Dong's stuff.  We generalize the method and propose online data integration that interleaves different components. 

\etitle{DR Evaluator.}  It evaluates the cleanness of the data in terms of data errors, and computes the benefit to apply data repairing by calling {\tt DR tools}. 

\etitle{EM Evaluator.}  It evaluates the cleanness of the data in terms of redundancy, and computes the benefit to apply entity matching by calling {\tt EM tools}. 

\etitle{EC Evaluator.}   It evaluates the cleanness of the cluster in terms of cluster uncertainty, and computes the benefit to apply entity consolidation by calling {\tt EC tools}. 

\etitle{Scheduler.}  It takes input a table $D$ and outputs a set of golden records $G$. It uses a small sample to decide whether to process DR first or EM first by calling DR evaluator and EM evaluator. 


\stitle{Possible Plans}


\etitle{EM $\rightarrow$ DR $\rightarrow$  EC}

\etitle{EM $\rightarrow$ DR $\rightarrow$  EM $\rightarrow$  EC}

\etitle{DR $\rightarrow$ EM $\rightarrow$ EC}

\etitle{DR $\rightarrow$ EM $\rightarrow$ DR $\rightarrow$EC}





\stitle{Cost Model for DR} For DR, we can use the number of changed clusters to evaluate DR. If we repair more tuples, the number does not change (or change a little), we do not need to ask more pairs. 


\stitle{Cost Model for EM} For EM, we can use the number of changed matching pairs (from matching to unmatching or from unmatching to matching) to evaluate EM. If we ask more pairs, the number does not change (or change a little), we do not need to ask more pairs. 

\stitle{Cost Model for EC} If the uncertainly of a cluster is low, i.e., we can simply use the majority voting to get a golden record, we do not need to ask.


\stitle{Cost Model for EM/DR Order}  Use a sample? If we cannot easily reach a consensus in a cluster, we need to do cleaning.  If there are duplicates, we need to first do entity matching. We need to do iterative EM and DR. 


Roughly speaking, it consists of two main components.

\stitle{Load/update/synchronize data.}
It serves two purposes.
(1) Update the information for the dataset, clusters and computed golden records.
(2) When there is an update of (1), which part of data should be recalculated (\eg block based, cluster based, and so on).

\stitle{Question scheduling.}
It decides that which questions from which module should be asked first.

\fi

%\nan{It seems that we have to revise each tool to be integrated in the framework, such that we can schedule the questions and reevaluation due to data update (\ie the ``'Exec'').}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%There are multiple ways to use the human operators and machine algorithms. For example, we can first use data cleaning operations, then entity matching operations and finally the data consolidation operations. We can also use entity matching operations, data cleaning operations and entity consolidation operations. We can also interleave  the three operations to achieve a much better consolidated results with much lower cost in terms of human interactions. The a nature question is that given a budget, how to find the best way to achieve the best performance. 

%This is to study that if interleaving the two processes of entity matching and entity consolidation,  we can achieve a much better consolidated results with much less cost in terms of human interactions.


\iffalse
The essential task of entity matching (EM) is to decide 
(1) which attribute values should be used; and
(2) how to decide the aligned attribute values are ``equal'' or very similar, syntactically or semantically.
%
Note that real-world data is often messy, including misspellings, missing values, various formats, and so on, which makes EM a hard problem. 
%
Entity consolidation (EC), on the other hand, is to find a ``preferred'' representation as given in Definition~\ref{def:ec}.

In practice, both EM and EC are time-consuming tasks, which need to heavily involve users (or crowd workers) to solicit many questions.

Assume that a user able to answer the following questions two given tuples $t_1$ and $t_2$:

\be
\itemsep-1mm\parsep-1mm
	\item $t_1$ and $t_2$ match based on attributes ${\cal A}$, where ${\cal A} \subseteq R$;
	\item[1'] $t_1[A_i] \preceq t_2[A_i]$, $A_i$ does not need to be in ${\cal A}$;
	\item $t_1$ and $t_2$ do not match; and
	\item some value $v$ in $t_1$ and $t_2$ should be $v'$.
\ee

Basically, users can do (1) if they know $t_1$ and $t_2$ based on which attribute set ${\cal A}$. Note that the attribute set ${\cal A}$ is tuple pair dependent; that is, different tuple pairs can match based on different attribute set.
%
(1') is tricky, but might be practical: if you see two persons with 10\% difference on weights, they might be the same person, but 30\% is probably a negative signal to say that they should not match. 
%
(2) is simple, that the user will say that these two tuples do not match. {\em Do the users need to say based on which attributes?}
(3) is a value update, which might to change a wrong value, or normalize some strings (\eg Prof. to Professor).

Assume that we give budget $B_1$ to the EM problem and $B_2$ to the EC problem, we may end up with a consolidated result, which we can measure precision and recall.

The hypothesis is, with the same budget $B_1 + B_2$, if we interleave EM and EC, we should achieve better precision and recall; or we achieve the same precision and recall using $B$ which is much less than $B_1 + B_2$.

\stitle{Why we can outperform?}
(1) Questions with indicated attributes are easy for users, but hard for machines.
(2) Batch string normalizations (or transformations) in the EC can make the EM much easier.
(3) ...?

We may also consider the following scenario later.

\begin{definition}
{\sc [Incremental Version.]} 
This means that the data is not static, where the new data $\Delta D$ will be inserted. Note that deletions are much rare than insertions, hence are not considered in this work.
\end{definition}
\fi


==> src/sec-algorithms.tex <==
%!TEX root = main.tex
\section{System Overview}
\label{sec:algorithms}






%For DR, we use the transformation rules to repair the data. To generate $Q_R$, we rank all the transformation-based repairs and select the top ones as candidate repairs.

%For EM, we have built the EM tools using the random forest.  To generate $Q_M$, we rank the pairs based on the similarity, and return the boundary pairs between the matching and unmatching pairs. 

%For EC, we just use the majority-voting based method.  To generate $Q_C$, we generate a question for each cluster.

%We will start to work on the algorithms details if most of us agree with the problem formulation. 

\iffalse
\subsubsection*{Challenges and Opportunities}

\be
	\itemsep-1mm\parsep-1mm

	\item How to generate questions for DR, EM, EC?

	\item How to allocate the budgets for DR, EM, EC?

	\item What is the optimization model?

	\item How to estimate the quality improvement? 
\ee
\fi


%\section{Conclusion}

==> src/sec-cor.tex <==
%!TEX root = main.tex
\section{Correlation-based Question Selection}
\label{sec:cor}

The previous method does not consider the correlation amongst different questions. For example, selecting two questions with the largest benefit might be worse than selecting two highly correlated questions, because correlated questions may have mutual positive influence on each other. To address this issue, we propose a correlation-aware question selection method. 


\subsection{Correlation on Two Dimensions}

We first consider whether two questions have correlations.  Given multiple questions, we first get the answers of these questions. Then we enumerate every two questions, run the machine algorithm, and compute the benefit of each question pair. Next we identify the question pair with the largest benefit improvement, and select the next questions from the two question sets. Iteratively this method can utilize the two dimension correlation to do question scheduling.

Note that this method requires to enumerate every two questions and it is expensive to run the machine algorithms $\mathcal{O}(N^2)$ times for $N$ questions. To address this issue, we have an observation that we can easily detect some questions have no correlations. Consider clustering questions and entity matching questions. They will generate more training data and have no positive correlation. Instead, they may have negative correlation. For example, if a clustering question covers an entity matching question (i.e., the cluster contains the two records of the entity pair), then they have negative correlation. Similarly, if a training rule question and a cluster question have large overlap on their records, they have negative correlation. In this case, we do not need to enumerate such question pairs. 

On the other hand, the entity matching question (training rule question, clustering question, entity matching question) may have positive  correlation with the data repairing question if one of them cannot improve the golden-record precision while they together can improve the golden-record precision. In this way, we can avoid enumerating the unnecessary question pairs and reduce the complexity of calling the machine algorithms. In addition, we can also select multiple questions (e.g., selecting $b$ questions in each round) in each time to reduce the number of calls to the machine algorithms.

\subsection{Correlation on Multiple Dimensions}

We then consider whether multiple questions have correlations. Here we use a-priori property to help us find correlations on multiple dimensions: if $Q_1, Q_2, \cdots, Q_i$ have no correlations, then for any question $Q_x$, $Q_1,Q_2, \cdots, Q_i, Q_x$ have no correlations. In this way, we can prune the searching space significantly. 

Next we discuss how to decide whether $Q_1, Q_2, \cdots, Q_i$ have correlations. If any $i-1$ size subset of $Q_1, Q_2, \cdots, Q_i$ has no correlation, we can deduce that $Q_1, Q_2, \cdots, Q_i$ has no correlation. Thus we assume any $i-1$ size of $Q_1, Q_2, \cdots, Q_i$ has correlations. Then we compute the benefit $\mathcal{B}_{Q_1, Q_2, \cdots, Q_i}$ of asking questions $Q_1, Q_2, \cdots, Q_i$, the benefit $\mathcal{B}_{\{Q_1, Q_2, \cdots, Q_i\}-Q_j}$ of asking questions $\{Q_1, Q_2, \cdots, Q_i\}-Q_j$, the benefit $\mathcal{B}_{Q_j}$ of asking question $Q_j$. 

If $\mathcal{B}_{Q_1, Q_2, \cdots, Q_i}>\max_{1\leq j\leq i} (\mathcal{B}_{\{Q_1, Q_2, \cdots, Q_i\}-Q_j}+\mathcal{B}_{Q_j}),$
then  $Q_1, Q_2, \cdots, Q_i$ have correlations, otherwise they have no correlations. 

For example, in Figure~\ref{fig:cor-example}, as the third 2-dimensional pair has no correlations, the second and third 3-dimensional pairs have no correlations either. Similarly, as the sixth 2-dimensional pair has no correlations, the second and fourth 3-dimensional pairs have no correlations either. Thus we only need to consider the first 3-dimensional pair and prune others.

%we want to know whether they have correlations. W
%e.g., \qt and \qm, and compare four cases. (1) We run the machine algorithms based on the answers of one questions (\qt or \qm). (2) We run the machine algorithms based on the answers of one questions (\qt or \qm). 

\begin{figure}[!t]
\begin{center}
\centering
\includegraphics[width=0.5\textwidth]{figs/cor.eps}
\vspace{-1.5em}
\caption{Question Correlation\label{fig:cor-example}}
\end{center}
\vspace{-1.5em}
\end{figure}





%\subsection{Correlation Estimation}


==> src/sec-cost.tex <==
%!TEX root = main.tex
\section{Cost-based Question Selection}
\label{sec:cost}

The benefit-based method neglects the fact that different questions have different difficulties to be answered by human. For example, a clustering question with small size should be easier than a clustering   question with large size. To address this problem, we propose to utilize user study to compute a cost model in order to quantify different questions (Section~\ref{subsec:cost:def}) and then give a cost-aware question selection method (Section~\ref{subsec:cost:select}).


\subsection{Cost Estimation} \label{subsec:cost:def}

We first qualitatively compare the cost of different questions and then present a quantitative model. 

%\hi{Entity Matching Question.} An entity matching question asks the human to verify a record pair and it is the easiest question among the four question types. We can take the cost of an entity matching question as a unit cost.


\hi{Training Rule Question.} A training rule will cover $|\qt|$ (e.g., 10) record pairs, and human will check the record pairs. Since most of the pairs satisfy the rule, human does not require to examine the pairs one by one and instead she can check many pairs together, and thus the cost of a training rule question $\qt$ is larger than 1 and smaller than $|\qt|$. Intuitively the larger $|\qt|$ is, the larger the cost is. 


\hi{Clustering Question.} A clustering question may cover many records, and human requires to check all the records and split them into different sub-clusters. Since most of the records belong to the same cluster, the cost of a clustering question $\qc$ is larger than 1 and smaller than $|\qc|$. Intuitively the larger $|\qc|$ is, the larger the cost is. 


\hi{Transformation Question.} A transformation question will cover  $|\qr|$ (e.g., 10)  records, and human requires to check the records and decide whether apply the transformation to the records. Since the records for the transformation may be different, the cost of a transformation question $\qr$ is larger than 1 and smaller than $|\qr|$. Intuitively the larger $|\qr|$ is, the larger the cost is. 


\hi{Question Cost Model.} Next we propose a cost model to quantify the cost of different questions. Intuitively, the cost of a question depends on the time used to answer a question. To this end, we use a user study to compute the cost model. We first get a set of questions with different sizes, ask the human to answer these questions and record the time. Next we use regression models to compute the cost model. We try different models, e.g., linear distribution, polynomial distribution, exponential distribution, logarithmic distribution, and we find that the cost follows the linear model and get the following cost functions. 
\begin{equation}
\mathcal{C}=\alpha |Q|+\beta
\end{equation}
\noindent where $\mathcal{C}$ is the cost of a question $Q$, $\alpha$ and $\beta$ are two parameters. 
For different question types, we only need to instantiate the two parameters. 



Based on our experimental results on user study, we get the following cost models
%\begin{equation}
%\mathcal{C}_M=|\qm|=1
%\end{equation}
\begin{equation}
\mathcal{C}(\qt)=\frac{|\qt|}{12}+\frac{11}{12}
\end{equation}
\begin{equation}
\mathcal{C}(\qc)=\frac{|\qc|}{15}+\frac{14}{15}
\end{equation}
\begin{equation}
\mathcal{C}(\qr)=\frac{|\qr|}{3}+\frac{2}{3}
\end{equation}



\subsection{Cost-based Selection}\label{subsec:cost:select}

We still iteratively select questions to ask.  From each question $Q$, we select the best question based on the normalized cost, $\frac{S(Q)}{\mathcal{C}(Q)}$. Then for each selected question from each question type, we ask human to label the answer, run the machine algorithm to compute the normalized benefit. We select the next question from the sets with the largest normalized benefit. We iteratively select the questions until the budget is used up.


%(1) For clustering, training question, the normalized score is $\frac{S(Q)}{\mathcal{C}}$. Then we can select questions following this order; (2)For repairing question, we compute normalized frequency $\frac{|Q|}{\mathcal{C}}$, and we select the questions in this order.


%with the most benefit. Then we ask the question and compute the net effect of asking the question compute the  compute the normalized benefit. 







==> src/sec-overview.tex <==
%!TEX root = main.tex

%\section{Holistic Data Integration}\label{sec:holistic}

%\nan{It seems that Section 3 is also for problem definition. We should reorganize Sections 2 and 3.}

%Our method first uses machine-learning based EM model to generate some clusters, and then uses majority voting (MV) to infer the golden records in each cluster. To improve the accuracy of golden records, we will generate some potential questions in EM and MV, select some high-quality questions to ask human, and re-run the EM and MV tools using the human feedbacks. Iteratively, the algorithm can generate the golden records. In this section, we first introduce the machine modules in Section~\ref{subsec:machine},  then present the human operations in Section~\ref{subsec:human}, and finally give an overview of our solution in Section~\ref{subsec:hybrid}.


\subsection{Machine Modules} \label{subsec:machine}

We utilize the following machine modules to help us compute golden records.




 %It can also use active learning to select some ``hard'' pairs that are hard to discriminate by the model (\eg the EM model return that the pairs have 50\% probability of matching pairs and 50\% probability of non-matching pairs), asks the human to check the pairs in order to get more training data and uses the training data to improve the training model.









%For example, Figure~\ref{fig:ex:1} shows an example. It first 
%Table~\ref{table:ex:naive} shows the results of the machine algorithms. We can see that the clusters generated are not correct and the golden values are not correct. 


\subsection{Human Operations} \label{subsec:human}


\begin{table}[!t]
\centering
\caption{Notations \label{table:notation}}
\begin{tabular}{|l|l|}\hline
Notation & Description \\ \hline
$P$ & A set of matching pairs\\\hline
$C$ & A set of clusters\\\hline
$\qt(\Qt)$ & A (set of) training rule question \\\hline
%$\qm(\Qm)$ & An (set of) entity matching question\\\hline
$\qc(\Qc)$ & A (set of) clustering question \\\hline
$\qr(\Qr)$ & A (set of) transformation question\\\hline
\Qall & $\Qall = \Qt\cup \Qc \cup \Qr$ \\\hline
\Qs & $\Qs\subset \Qall$: seleceted questions \\\hline
$\mathcal{C}_T$ & The cos of training rule question $\qt$ \\\hline
%$\mathcal{C}_M$ & The cos of entity matching question $\qm$ \\\hline
$\mathcal{C}_C$ & The cos of clustering question $\qc$ \\\hline
$\mathcal{C}_R$ & The cos of transformation question $\qr$ \\\hline
\end{tabular}
\end{table}


We utilize the following human operations to improve entity matching and entity consolidation.

\subsubsection{Training Rule Question} 

To improve entity matching, we can use training rules to get more training data and feed them to the entity-matching tool to improve the EM  quality. However it is hard to get 100\% accurate rules and we ask human to validate the rules. If the rules are approved, we take the record pairs that satisfy the rule as training data and re-train the EM model; otherwise we skip the rule.

\hi{Training Rule Validation Question.} Formally, a matching (non-matching) rule question $\qt$ includes an ``if-condition-then-matching (non-matching)'' clause as well as several records pairs that satisfy the rule.  For example, $Jaccard(Name)\ge 0.5$ is a matching rule and $Jaccard(Address)\le 0.1$ is a non-matching rule. To help human validate a training rule, we also associate a sample of entity pairs  that satisfy the rules (\eg 10 pairs).  We use \qt to denote a training rule and \Qt to denote a set of training rules.




\hi{Training Rule Generation.} The training rules can be hand-crafted by domain experts or the rules learned from random forest (i.e., the leaf nodes in the random forest). 

For example, Table~\ref{fig:tr:ex} shows 3 training rule examples. The rule {\it if the same Zipcode then matching} will take all the records with the same Zipcode as matching pairs.


\begin{figure}[!t]
\begin{center}
\centering
\begin{tabular}{|p {12em} | p {8em} |l|}\hline
Training Rule & 3 examples & Results \\ \hline
If $Jaccard(\texttt{Name})\ge 0.5$ then Matching & $(r_1,r_2), (r_3, r_4)$, $(r_5, r_6)$& Yes\\\hline
If $Jaccard(\texttt{Address})\ge 0.5$ then Matching & $(r_1,r_2), (r_3, r_4)$, $(r_7, r_8)$& Yes\\\hline
If same $\texttt{Zipcode}$ then Matching & $(r_1,r_2), (r_1, r_7),$ $(r_7, r_8)$& Yes\\\hline
\end{tabular}
\vspace{-.5em}
\caption{Training Rules\label{fig:tr:ex}}
\end{center}
\vspace{-1.5em}
\end{figure}





%%%%%%%%%%%Remove EM questions%%%%%%%%%
\iffalse

\subsubsection{Matching Pair Validation} 

To improve entity matching, we can use active learning to select entity pairs, ask the human to validate the pairs, and feed them to the entity matching tool to improve the matching quality. 

%We require to ask the human to validate the pairs. 


\hi{Entity Matching Validation Question.}  Formally, an entity matching question $\qt$ is a pair of records. We ask human to verify whether the pair refers to the same entity. Then the result is taken as the training data. Obviously $|\Qm|=1$.


\hi{Entity Matching Question Generation.} All the pairs can be taken as an entity matching question. However there are huge number of pairs. To address this problem, we can use active learning to select record pairs. The basic idea is that for each record pair, it utilizes the entity matching tool to compute a probability whether the pair is a matching pair. If the probability is close to 0.5, the entity matching tool cannot  discriminate it and will take it as an entity matching question. We will introduce the details in Section~\ref{sec:benifit}.

%Based on the matching pairs returned by the entity matching tool, we can compute a similarity threshold that is around the matching pairs and non-matching pairs. For each pair, we compute a similarity, which is the average similarity on each attribute. We can use any similarity functions, e.g., Edit distance, Jaccard. Then we take the smallest threshold among all the pairs as the similarity bound. Then we can select the top pairs smaller than the bound as matching questions. 

For example, the EM tool cannot discriminate $\langle r_5, r_6\rangle$ clearly and we want to ask this pair to train a more effective model. 

\fi 
%%%%%%%%%%%Remove EM questions%%%%%%%%%



\begin{figure}[!t]
\begin{center}
\centering
\begin{tabular}{|l | l |}\hline
Cluster & Results \\ \hline
\{$r_1,r_2,r_3,r_7,r_8$\} & No: $\{r_1,r_2,r_3\}$; \{$r_7,r_8$\}\\\hline
\{$r_4,r_5,r_6$\} & No: $\{r_4\}$; \{$r_5,r_6$\}\\\hline
$\{r_5,r_6,r_7,r_8\}$ & Yes \\\hline

\end{tabular}
\vspace{-.5em}
\caption{Cluster Questions\label{fig:tr:ex}}
\end{center}
\vspace{-1.5em}
\end{figure}



\subsubsection{Clustering Question} 

The EM model may generate incorrect clusters. To improve the cluster quality,  we can ask human to verify a cluster of records. If the records in the cluster do not refer to the same entity, human is required to split the records in the cluster into several sub-clusters where all records in each sub-cluster refer to the same entity; otherwise, all the records in the cluster are validated to be matching.


\hi{Clustering Validation Question.}  Formally, a clustering question $\qc$ is a cluster of records. We ask   human to verify whether the pairs in the cluster refer to the same entity. If the records do not refer to the same entity, the human requires to spilt the cluster into $C_1, C_2,\cdots, C_y$ clusters.  Then the pairs in the same cluster can be taken as matching pairs and the pairs from different clusters can be taken as non-matching pairs, and these validated pairs will be taken as the training data to feed the EM model.  We use \qc to denote a clustering question and \Qc to denote a set of clustering questions.


\hi{Clustering Question Generation.}  All the clusters generated by the EM model can be taken as a cluster question. 

For example, Table~\ref{fig:tr:ex} shows 3 clustering questions.  Cluster \{$r_1,r_2,r_3,r_5,r_7,r_8$\} in Figure~\ref{fig:ex:1} can be chosen as a cluster question, and human can discriminate the address of MIT EECS from MIT Computer Science, and split the cluster into two sub-clusters: one for EECS and the other for Computer Science. 


\begin{figure}[!t]
\begin{center}
\centering
%\includegraphics[width=0.5\textwidth]{figs/gr-example.eps}
\begin{tabular}{|l|l|l|}\hline
Transformation Rule & 3 Examples & Results  \\ \hline
\#th $\rightarrow$ \# (\# is a numerical value) & $r_3,r_5,r_7$ & Yes\\\hline
Street $\rightarrow$ St & $r_4,r_8$ & Yes\\\hline
\end{tabular}
\vspace{-.5em}
\caption{Transformation Rules\label{fig:gr-example}}
\end{center}
\vspace{-1.5em}
\end{figure}



\subsubsection{Transforamtion Rule Question} 

Since the data is dirty or has different representations,  in many cases there may not exist majority values in an attribute, and it requires to normalize/repair the data to improve the quality of golden records. Here we use the transformation rule as an example to repair the data. A rule $v\rightarrow v'$ repairs the records with value $v$ to the value $v'$. We can ask human to validate the rule. If the rule is approved, we use the rule to transform the data; otherwise we skip the rule.  


\hi{Transformation Validation Question.}  Formally, a transformation validation question $\qr$ is a transformation rule $v\rightarrow v'$ as well as a sample of records with value $v$. We ask the human to verify whether repairing rule can be applied to the records. If the rule is approved, we pair the records and update the dataset $D$. For example, Figure~\ref{fig:gr-example} shows several transformation rules. \#th(nd) $\rightarrow$ \# will transform a numerical value with th(nd) to the numerical value, e.g., 50th to 50 and 32nd to 32.


 %Here $|\Qr|$ is the number of records in the rule. %We ask the human to identify the records that can be applied for the rule. 
% consider three repairing rules: ${Capital[2]}digit[+] \to {Capital[2]}$ can be applied to $MASSACHUSETTS \to MA$ and $CALIFORNIA \to CA$. Rules $Avenue \to Ave$ and $boulevard \to blvd$ can be applied to the street column.

\hi{Transformation Question Generation.}  For each cluster, on each attribute, we align the attribute values as follows. We first get some matching tokens and then split the attribute value based on the matching tokens and generate some segments. Then for each segment pair $(v, v')$, we generate a transformation  rule. We can also group the transformation rules for different pairs and each transformation rule includes all the corresponding records containing $v$. 
%Thus $|\qr|$ is the size of records associated with the rule \qr. 
Please refer to \cite{DBLP:journals/corr/abs-1709-10436} for more details of transformation rule generation. 
 We use \qr to denote a transformation rule and \Qr to denote a set of transformation rules.


%For example, Figure~\ref{fig:gr-example} shows several transformation rules.



\subsection{Human-in-the-loop Data Integration} \label{subsec:hybrid}


%Given a set of training rule questions \Qt,  a set of clustering questions \Qc, and a set of transformation questions \Qr,  and 
%For each question, it asks human to get the answers, runs the machine algorithms, and asks the next questions. Iteratively, it can get the golden records. 

Initially, we need to run the machine algorithms to generate question sets \Qt, \Qc, and \Qr. Toward this goal, we require to get some training data to train the EM model. We select several training rules to get such training data (we will discuss the details on how to select training rule questions in Section~\ref{subsec:sorting}). Then we run the machine algorithms to generate the clusters and infer the golden records. In this way, we can generate three sets of questions, $\mathbb{Q}_T$, $\mathbb{Q}_C$, and  $\mathbb{Q}_R$.  Let $\Qall = \Qt\cup \Qc\cup \Qr$ denote the set of all possible questions. 


Given a budget to ask human, we aim to select a sequence of questions $\Qs=\langle Q_1,Q_2, \cdots, Q_B\rangle$ to ask human in order to maximize  the accuracy of golden records, where $Q_i$ is either a training rule question, clustering question or transformation question. A brute-force question scheduling method enumerates every $B$-size permutation of $\Qall$, computes the golden-record quality (after asking these questions, getting answers, and re-running the machine algorithms), and selects the permutation with the largest quality as \Qs. However this method has several challenges.

\hi{Challenge 1: Question Sequence Enumeration.} It is prohibitively expensive to enumerate all permutations of $B$-size subsets of $\Qall$.

\hi{Challenge 2: Golden-record Qualtiy Computation.} It is rather hard to compute the golden-record quality of a question sequence, because $(i)$ we do not know the ground truth of golden records, and $(ii)$ we do not know the human answer of each question before we ask the questions. 


\hi{Challenge 3: Questions have correlations.}  Asking a question may affect the clusters and golden records, and thus affect other questions. So \Qall will dynamically changes after asking some questions. We cannot select a static set of questions \Qs in a single round. Instead, we aim to first select several questions, use the human feedback of these questions to compute the clustering quality and golden-record quality, and then utilize the results to guide us to select the following questions. 


To address the above challenges, we propose an iterative estimation based method. The basic idea is that it selects $b$ questions in each round, uses the human feedback of these $b$ questions to estimate the benefit of each question (and a question sequence), and then utilizes the benefits to select $b$ questions in next round. We will present the details in the next section.





%It is rather hard to compute the golden-record quality of a question sequence, because $(i)$ we do not know the ground truth of golden records, and $(ii)$ we do not know the human answer of each question before we ask the questions. 






















\iffalse
We first use several matching training rules and non-matching training rules to get some training data. Next we run the machine algorithms to generate the golden records. Then we can get four sets of questions, $\mathbb{Q}_T$, $\mathbb{Q}_M$,  $\mathbb{Q}_C$, and  $\mathbb{Q}_R$. 
Next we select some questions from the four question sets, ask the human to get the results, and generate some training data (for questions in $\mathbb{Q}_T$, $\mathbb{Q}_M$,  $\mathbb{Q}_C$) and repair the dataset $D$ (for questions in $\mathbb{Q}_R$).  Next we call the machine algorithms using the new training data and the updated  datasets. We repeat the above steps until the budget is used up. Finally we can get the set $G$ of golden records.

\lgl{add pseudo code here}

\lgl{refine the examples}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]\vspace{-1em}
\begin{center}
\centering
\includegraphics[width=0.5\textwidth]{figs/odi4.eps}
\vspace{-1.5em}
\caption{Question Selection Framework\label{fig:arch4}}
\end{center}
\vspace{-1.5em}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

One big challenge here is to select ``high-quality'' questions.  A straightforward way selects questions in a round-robin strategy, i.e., select one question for each question type in each iteration.  However this method cannot work well, because different questions have different cost and benefit. For example, training rule questions, entity matching questions and clustering question can improve the cluster quality, while the date-repairing question can improve the golden record accuracy. Thus, we need to judiciously select questions to maximize the golden-record quality.  Figure~\ref{fig:arch4} shows the framework of question scheduling and Figure~\ref{fig:rex} shows a running example. \ji{ [Ji modified] Initially, we know nothing about the cluster, tuples are separated completely, in this case, the best choice is using validated rule to improve the recall of the cluster. After applying rule Jaccard(street) $\ge$ 0.5, $r_{9}, r_{10}$ are incorrectly classified into the first cluster as their addresses are too close to tuples in the first cluster. There are three errors now, we can not reduce rule threshold to connect $r_{9}r_{11}$ or $r_{5}r_{6}$ because that would bring more harm than benifits, and we can not ask repairing question because nonsense questions like $77\to1400$ would be chose as repairing question at this moment. Therefore, we choose cluster question to split $r_{9}$ and $r_{10}$ from the first cluster. All the university names and their abbreviations appear in same clusters now, and we can repair all these in one slot by asking repairing question, the red circles indicate the tuples whose name is modified. Machine will connect $r_5$ and $r_6$ because of same name. At last, add validated rule Jaccard(name) $\ge$ 0.5 to connect $r_9$ and $r_{11}$ and add them into training data to train new model.} $r_{5}, r_8$ should be merged with $r_6$ and $r_7$. $r_9, r_{10}$ should be merged with $r_{11}$ and $r_{12}$. Then in the first round, we select a cluster question $Q_C$ for cluster \{$r_1,r_2,r_3,r_4, r_{17}, r_{18}$\}, and it is split into two clusters  \{$r_1,r_2,r_3,r_4$\} and \{$r_{17}, r_{18}$\}. Then the EM tool classifies $r_{17}, r_{18}$ into the clusters of $r_{19}$ and $r_{20}$. Then the clusters  \{$r_1,r_2,r_3,r_4$\} and  \{$r_{15}, r_{16}, r_{17}, r_{18}$\} are correct. Next in the second round, we select an EM question $Q_M$ for asking whether $r_5$ and $r_6$ refer to the same entity.  Then the EM tool merges $r_5, r_8$ and $r_6,r_7$ and gets a correct cluster. In the third round, we ask a data repairing question \texttt{California$\leadsto$ CA}, and the machine algorithm merges $r_9, r_{10}$ and $r_{11},r_{12}$ and gets a correct cluster and correct golden value.


\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]\vspace{-1em}
\begin{center}
\centering
\includegraphics[width=0.5\textwidth]{figs/rex.eps}
\vspace{-1.5em}
\caption{Running Example for Question Scheduling\label{fig:rex}}
\end{center}
\vspace{-1.5em}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
\fi

%\lgl{add an example}
%the records do not refer to the same entity, the human requires to spilt the cluster into $c_1,c_2,\cdots, c_y$ clusters.   Then the pairs in the same cluster can be taken as matching pairs and the pairs from different clusters can be taken as non-matching pairs, and these results are taken as the training data. Here $|\qc|$ is the number of records in the cluster.





==> src/sec-removed.tex <==

















%We made the following observations. 






%\benefit method achieved the best accuracy and outperformed other methods by more than 10 percent, because \benefit  can judiciously select questions to ask.  \qronly outperformed other methods, because simply majority voting cannot get high-quality golden records and \qronly can transform the data based on the transformation rules.  However \qronly was worse than \benefit, because the clusters had no 100\% accuracy and it required to use other questions to improve the clustering quality. . Secondly, with the increase of the number of questions, \benefit consistently improved the accuracy and other methods cannot be improved after asking some questions, because \benefit judiciously selected questions while otherwise only asked a fixed group questions. For example, on the \addr dataset, \benefit consistently improved until asking 50 questions while \qronly was stable after asking 30 questions, \qmonly and \qconly were stable after asking 10 questions. Thirdly, all the methods had lower quality on the \pub dataset, because the dataset was more dirty than others. 



%igure shows the results. We can see that local ranking took much higher time than other components, because it needed to compute the uncertainty for many pairs.
%was efficient as it only needed to process the 
%\lgl{x: k, cost=100?}




%Secondly, \qconly, \qronly, \qtonly, and \random. 
%were better than the non-interleaving methods, \emec, \qconly, \qronly, \qtonly, %\lgl{Add a latency figure}



%Secondly,  \globalkcorrtwo and \globalkcorrfour achieved similar performance, because both of them considered correlations. 



%we could also use batching-based technique on correlations and we could see that  \corr-5 (selecting 5 questions in each round) was slightly worse than the non-batching method \corr-1 (selecting 1 question in each round), but \corr-5 could reduce the latency.

%with a larger $b$, the GR accuracy become slightly lower, because it needed to select $b$ questions in each round and could not use more previous information to select better questions. However it could reduce the time cost of machine algorithms. Secondly, it was tradeoff to use a batching-based method. If the user did not care about the latency of the machine algorithms, she can use the non-batching method to get much better results. On the contrary, the user could reduce the latency at a little cost of quality. Figure~\ref{fig:latency:cost} showed the latency. We could observe that \costaware-b could reduce a lot of latency compared with \costaware-1.






%We compared the correlation-based method \corr and the cost-aware benefit method \nocorr (without correlation). Figure~\ref{fig:gr:cor} showed the results. We made the following observations. Firstly, the correlation-based method could improve the GR accuracy by 3-5\%, because it could use correlation to select the questions and there indeed existed correlations between entity matching questions and transformation questions. Secondly, we could also use batching-based technique on correlations and we could see that  \corr-5 (selecting 5 questions in each round) was slightly worse than the non-batching method \corr-1 (selecting 1 question in each round), but \corr-5 could reduce the latency.

%\lgl{add latency results}






%\subsection{Evaluation on Different EC Methods}

%We also evaluated different EC methods and showed that our method could improve the GR accuracy for different EC techniques. 






















%compare \cost-1 vs \cost-5, \cost-10

%x: different methods with different cost functions? 
%y: golden-record accuracy



% \hi{Clustering Quality.} We also evaluated the clustering quality by varying the cost. Figure~\ref{fig:f1:cost} showed the results. We had the following observations. Firstly, \costaware still outperformed other methods, because it could selected a mixed set of questions to ask. Secondly, \qconly, \qmonly, and \qtonly outperformed \qronly, because the former three aimed to improve clustering quality while \qronly could only transform the data. Thirdly,  \qconly and \qmonly were better than \qtonly, because it was not easy to find 100\% accurate training rules and it was expensive to ask many pairs of a training rule, while \qconly and \qmonly could ask more ``beneficial'' clusters and pairs to ask using active learning to improve the clustering quality. Fourthly, \qconly was better than \qmonly in the beginning because the normalized benefit of a clustering question was better than an EM question; while after asking more questions, the clusters had higher quality and it was hard to improve the clustering accuracy.

%the methods can improve the GR accruacy  Secondly, Thirdly. Compare \qtonly, \qmonly, \qconly, \qronly, \benefit,



%x: question noy: golden-record accuracy

%x: question no y: clustering quality



%the Compare \qtonly, \qmonly, \qconly, \qronly, \cost,

%x: cost
%y: golden-record accuracy



%\cost, \corr

%x: cost
%y: golden-record accuracy


%\hi{Batching vs Non-Batching.} We also compared the batching-based methods \corr-5 (selecting 5 questions in each round), \corr-10 (selecting 10 questions in each round), and the non-batching method \corr-1 (selecting 1 question in each round). Figure~\ref{} showed the results. We made the following observations. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse




%Secondly, the repairing questions had the largest cost, because in each transformation rules there were many records that satisfied the rule, and as these records were quite different, the users were required to go through the records to validate whether applying the rule. But for clustering questions, the records in the cluster were very similar, the users could very easily to validate a cluster (and a training rule). 

% \lgl{add a figure, x: question size, y: time}



%benefit-based method and assumed that different questions had the same cost. We varied the number of questions and compared the golden-record accuracy of different methods. Figure~\ref{fig:gr:no} showed the results. 

\subsection{Cost-Aware Benefit-Based Method}

We evaluated different cost model and compared the cost-aware benefit-based methods. 



\hi{Cost-Aware Question Selection.} We compared different methods by considering the normalized benefit based on the cost. We varied the cost and Figure~\ref{fig:gr:cost} on the GR accuracy. Note that in the figure, the cost of ``100'' means if only asking EM questions, there were 100 question; if only asking clustering questions, there were about 7 questions; if only asking GR questions, where were about 30 questions. We had the following observations. 

Firstly, the normalized benefit method \costaware still achieved the highest GR accuracy, because \costaware considered the cost of different questions and judiciously selected questions to ask.  Secondly, \qmonly achieved higher performance than \qronly and then was worse than \qronly, because \qmonly had lower cost than other questions and could improve the clustering quality at the beginning and when the clustering quality was high enough and cannot be improved, \qmonly cannot improve the golden-record accuracy anymore; while \qronly can consistently improve the golden-record accuracy by repairing the data. Thirdly, \qronly could improve the GR accuracy with the increase number of cost, as it could transform more data while \qconly and \qtonly could only improve the clustering quality. Fourthly, all the methods had low quality on \pub dataset because it was more dirty than other two datasets. 

\hi{Clustering Quality.} We also evaluated the clustering quality by varying the cost. Figure~\ref{fig:f1:cost} showed the results. We had the following observations. Firstly, \costaware still outperformed other methods, because it could selected a mixed set of questions to ask. Secondly, \qconly, \qmonly, and \qtonly outperformed \qronly, because the former three aimed to improve clustering quality while \qronly could only transform the data. Thirdly,  \qconly and \qmonly were better than \qtonly, because it was not easy to find 100\% accurate training rules and it was expensive to ask many pairs of a training rule, while \qconly and \qmonly could ask more ``beneficial'' clusters and pairs to ask using active learning to improve the clustering quality. Fourthly, \qconly was better than \qmonly in the beginning because the normalized benefit of a clustering question was better than an EM question; while after asking more questions, the clusters had higher quality and it was hard to improve the clustering accuracy.



\begin{figure*}[!t]
 \begin{center}
 \subfigure[Address]{
     \label{subfig:gr:no:address}
     \includegraphics[width=0.3\textwidth]{exp/figure1/address-gr.eps}
 }
 \subfigure[Products]{
     \label{subfig:gr:no:product}
     \includegraphics[width=0.3\textwidth]{exp/figure10/big-products-gr.eps}
 }
 \subfigure[Publication]{
     \label{subfig:gr:no:pub}
     \includegraphics[width=0.3\textwidth]{exp/figure1/publication-gr.eps}
 }
 \end{center}
\vspace{-1.5em}
 \caption{GR Accuracy by Varying Question Number \label{fig:gr:no}}
\vspace{-1em}
%\end{figure*}
%\begin{figure*}[!ht]
 \begin{center}
 \subfigure[Address]{
     \label{subfig:f1:no:address}
     \includegraphics[width=0.3\textwidth]{exp/figure4/address-cluster.eps}
 }
 \subfigure[Products]{
     \label{subfig:f1:no:product}
     \includegraphics[width=0.3\textwidth]{exp/figure12/big-products-cluster.eps}
 }
 \subfigure[Publication]{
     \label{subfig:f1:no:pub}
     \includegraphics[width=0.3\textwidth]{exp/figure4/publication-cluster.eps}
 }
 \end{center}
\vspace{-1.5em}
 \caption{Clustering Quality by Varying Question Number   (F1 Measure) \label{fig:f1:no}}
\vspace{-1em}
\end{figure*}


\begin{figure*}[!t]
 \begin{center}
 \subfigure[(4+size)/5]{
     \label{subfig:gr:func:addr:5}
     \includegraphics[width=0.3\textwidth]{exp/figure6/address-cost-5.eps}
 }
 \subfigure[(9+size)/10]{
     \label{subfig:gr:func:addr:10}
     \includegraphics[width=0.3\textwidth]{exp/figure6/address-cost-10.eps}
 }
 \subfigure[(99+size)/100]{
     \label{subfig:gr:func:addr:100}
     \includegraphics[width=0.3\textwidth]{exp/figure6/address-cost-100.eps}
 }
 \end{center}
\vspace{-1.5em}
 \caption{GR Accuracy by Varing Cost Functions (\addr) \label{fig:gr:func:addr}}
\vspace{-1em}
\end{figure*}
 
 
\begin{figure*}[!t]
 \begin{center}
 \subfigure[(4+size)/5]{
     \label{subfig:gr:func:product:5}
     \includegraphics[width=0.3\textwidth]{exp/figure6/address-cost-5.eps}
 }
 \subfigure[(9+size)/10]{
     \label{subfig:gr:func:product:10}
     \includegraphics[width=0.3\textwidth]{exp/figure6/address-cost-10.eps}
 }
 \subfigure[(99+size)/100]{
     \label{subfig:gr:func:product:100}
     \includegraphics[width=0.3\textwidth]{exp/figure6/address-cost-100.eps}
 }
 \end{center}
\vspace{-1.5em}
 \caption{GR Accuracy by Varing Cost Functions(\product, todo) \label{fig:gr:func:product}}
\vspace{-1em}
\end{figure*}

\begin{figure*}[!t]
 \begin{center}
 \subfigure[(4+size)/5]{
     \label{subfig:gr:func:pub:5}
     \includegraphics[width=0.3\textwidth]{exp/figure6/address-cost-5.eps}
 }
 \subfigure[(9+size)/10]{
     \label{subfig:gr:func:pub:10}
     \includegraphics[width=0.3\textwidth]{exp/figure6/address-cost-10.eps}
 }
 \subfigure[(99+size)/100]{
     \label{subfig:gr:func:pub:100}
     \includegraphics[width=0.3\textwidth]{exp/figure6/address-cost-100.eps}
 }
 \end{center}
\vspace{-1.5em}
 \caption{GR Accuracy by Varing Cost Functions(\pub, todo) \label{fig:gr:func:pub}}
\vspace{-1em}
\end{figure*}



%x: cost y: clustering quality


\hi{Varying Different Cost Functions.} 
We also tried different cost functions. Figures~\ref{fig:gr:func:addr}, \ref{fig:gr:func:product}, and \ref{fig:gr:func:pub} showed the results. We made the following observations. Firstly, with different cost functions, \costaware still achieved the best performance and worked well for different cost functions. Secondly, with larger division ratio, \qtonly, \qconly and \qronly achieved better results, because their cost become smaller for larger division ratio. 


\hi{Batching vs Non-Batching.} We compared the batching-based method, e.g., \costaware-b (selecting $b$ questions in each round) and the non-batching method \costaware-1 (selecting 1 question in each round). Figure~\ref{fig:cost:batch} showed the results. We made the following observations. 
Firstly, with a larger $b$, the GR accuracy become slightly lower, because it needed to select $b$ questions in each round and could not use more previous information to select better questions. However it could reduce the time cost of machine algorithms. Secondly, it was tradeoff to use a batching-based method. If the user did not care about the runtime of the machine algorithms, she can use the non-batching method to get much better results. On the contrary, the user could reduce the latency at a little cost of quality. Figure~\ref{fig:latency:cost} showed the latency. We could observe that \costaware-b could reduce a lot of latency compared with \costaware-1.

\begin{comment}
\begin{figure*}[!t]
 \begin{center}
 \subfigure[Address]{
     \label{subfig:gr:cost:address}
     \includegraphics[width=0.3\textwidth]{exp/figure2/address-cost-gr.eps}
 }
 \subfigure[Products]{
     \label{subfig:gr:cost:product}
     \includegraphics[width=0.3\textwidth]{exp/figure2/products-cost-gr.eps}
 }
 \subfigure[Publication]{
     \label{subfig:gr:cost:pub}
     \includegraphics[width=0.3\textwidth]{exp/figure2/publication-cost-gr.eps}
 }
 \end{center}
\vspace{-2em}
 \caption{GR Accuracy by Varying Cost \label{fig:gr:cost}}
\vspace{-1.5em}
 \begin{center}
 \subfigure[Address]{
     \label{subfig:f1:cost:address}
     \includegraphics[width=0.3\textwidth]{exp/figure5/address-cost-cluster.eps}
 }
 \subfigure[Products]{
     \label{subfig:f1:cost:product}
     \includegraphics[width=0.3\textwidth]{exp/figure13/big-products-cost-cluster.eps}
 }
 \subfigure[Publication]{
     \label{subfig:f1:cost:pub}
     \includegraphics[width=0.3\textwidth]{exp/figure5/publication-cost-cluster.eps}
 }
 \end{center}
\vspace{-1.5em}
 \caption{Clustering Quality by Varying Cost  (F1 Measure) \label{fig:f1:cost}}
\vspace{-1em}
\end{figure*}
\end{comment}

\fi




\begin{comment}
\begin{figure*}[!t]
 \begin{center}
 \subfigure[Address]{
     \label{}
     \includegraphics[width=0.3\textwidth]{exp/figure14/address-cost-gr.eps}
 }
 \subfigure[Products]{
     \label{}
     \includegraphics[width=0.3\textwidth]{exp/figure14/products-cost-gr.eps}
 }
 \subfigure[Publication]{
     \label{}
     \includegraphics[width=0.3\textwidth]{exp/figure14/publication-cost-gr.eps}
 }
 \end{center}
\vspace{-1.5em}
 \caption{GR Accuracy by Varying k\label{fig:gr:k}}
\vspace{-2em}
\end{figure*}
\end{comment}


\iffalse
\begin{figure*}[!t]
 \begin{center}
 \subfigure[Address]{
     \label{}
     \includegraphics[width=0.3\textwidth]{exp/figure15/address.eps}
 }
 \subfigure[Products]{
     \label{}
     \includegraphics[width=0.3\textwidth]{exp/figure15/products.eps}
 }
 \subfigure[Publication]{
     \label{}
     \includegraphics[width=0.3\textwidth]{exp/figure15/publication.eps}
 }
 \end{center}\vspace{-1.5em}
 \caption{Machine Time For Different Size\label{fig:latency}}
\vspace{-1em}
\end{figure*}
\fi


%For the two datasets with 1 million records, our method only takes 20 minutes. %, using parallel and incremental techniques.


%Due to the page limit of the response letter, we simplify and group some comments of the meta reviewer.
%that have overlaps with the ones from the previous three reviewers. 
%As the ground truth of golden records are unknown, we propose 


%Then we ask the cluster questions in a bottom-up manner. For each leaf node, we take the cluster as a question. If the cluster is not split (e.g., all the records in the cluster refer to the same entity), we select a record and put the record into its parent node; other we remove the node from its parent. We repeatedly ask the cluster the question until reaching the root node. 


%a new hierarchical clustering method, which each node in the hierarchical cluster has the same number of children (e.g., 10). 

% if the global benefit of a question has been computed in previous iterations, we can just utilize this global benefit as an estimation and do not need to recompute it from scratch.
 
%$(2.1)$ Local Ranking.  $(2.1.1)$ Training Question. We can compute the score of each training rule in parallel.  $(2.1.2)$ Cluster Question. We computed score of each candidate cluster in parallel.  $((2.1.3)$ Transformation Question.  We can split the records into different partitions, compute the transformation rule for each partition and then merge the transformation rule. $(2.2)$ Global Ranking. We compute the global score of each local question generated from local ranking in parallel for $b = 1$. For $b = 2$, we compute the score for each local question pair in parallel. For $b>2$, we first group the questions and compute the score of each group in parallel.


% $(1)$ {\it Incremental Computing.}  We propose incremental computing techniques to accelerate our method.  $(1.1)$ Local Ranking.  $(1.1.1)$ Training Question. First, we do not need to recompute the coverage and accuracy in each round; instead we only need to check the records that have been updated by the transformation questions in the previous round. Second, as we compute top-$k$ training questions, we can use a priority queue to keep the $k$ best questions, maintain an upper bound for these questions, and use the upper bound to prune the training questions that cannot be in the top-$k$ list.  $(1.1.2)$ Cluster Question.  We still use a priority queue to keep the $k$ best questions, maintain an upper bound for these questions, and use the upper bound to prune the questions that cannot be in the top-$k$ list.  The upper bound is calculated based on the cluster size and maximal utility.  $(1.1.3)$ Transformation Question. Instead of generating all the transformation rules from the dataset up-front, we can generate the transformation rule with the largest frequency in each round. For this purpose, we first partition the value pairs based on their syntactical structures (for example, 5th-->5 and 20th-->20 will be in the same partition). Then, the size of the partition can serve as an upper bound for the frequency of the transformation rules generated from this partition. Since we only generate the ``best transformation rule'' with the largest frequency in each round, we can visit the partitions in their size order, generate transformation rules in each partition, and terminate whenever the current partition size is smaller than the frequency of the best transformation rule we found so far. 









%  Indeed, in every round we use the results of previous rounds to improve our model. In the extreme case, with batch size 1, we are doing exactly active learning. However, we improve this extreme case by interleaving multiple questions in each round to capture the question correlation. Note that improving the matcher can only improve the clustering quality while our approach not only improves the matcher but also transforms variant values into canonical values in order to generate the golden records.

%The size of each cluster is not large, and is usually smaller than the number of data sources. In particular, we have been working with a major data integration company that deals with several hundred customers for entity matching and consolidation tasks -- no customer has more than 100 data sources and the cluster size never exceeds 100. Therefore, cluster questions can be handled by humans. In fact, in the extreme case of large clusters, we will not select the large clusters since they have large human costs and small benefit/cost ratio. Even if the selected cluster is still large, sampling records within clusters works pretty well in practice.

%\ji{[If large clusters exist, we can split each cluster into several smaller clusters by using k-means or other unsupervised clustering methods and generate easier questions from them.]}



% We will include these new results in the paper.  We have evaluated our method on two large datasets, each with 1 million records. Our method only asks ~600 questions (10 questions per round for 60 rounds). In each round, the machine time is 20 seconds and the human time is around 2 minutes. In total, our method only takes 2.5 hours to process 1 million records. Second, the human effort is scalable. Note that each worker can answer any training/cluster/transformation question, without waiting upon each other. Also, the human effort can be further improved if there are more workers, e.g., using crowdsourcing. Moreover, the number of questions is not proportional to the number of records. In principle, it is determined by the number of questions/answers needed to capture the characteristics of the datasets, including training questions for entity matching, cluster questions for cluster debugging, and transformation questions for entity consolidation. Thus our method only needs to ask hundreds of questions for 1 million records.  Third, the machine algorithms are also scalable through parallelization and incremental computing. For the two datasets with 1 million records, our method only takes ~20 minutes, using parallel and incremental techniques. We will include these new results in the paper. 


% $(ii)$ {\it Parallel Computing Techniques.}   Firstly, The change of local ranking score for the training questions happens only when some tuples in the data changes by transformation rules, so we can recalculate the score by adding or removing the effect of transformed records incrementally. Secondly, the local score of cluster questions are more complicated because that it's related to the matcher, however, we can still get tighter lower bound of cluster size and $Pr(p)$ with program going. Thirdly, we incrementally choose the best transformation group among all possible transform pairs.


%We have conducted new experiments on two large datasets, each with 1 million records, and the new results are shown in Section~\ref{}.  Our method only asks ~600 questions (10 questions per round for 60 rounds). In each round, the machine time is 20 seconds and the human time is around 2 minutes. In total, our method only takes 2.5 hours to process 1 million records. 



%\ji{Parallel Techniques: Firstly, Before training matcher, we extract features of candidate pairs in parallel. Secondly, When global ranking questions by benifits, we compute benifits entropy of questions in parallel. Thirdly, when local ranking, we compute the local score of training rule questions and cluster questions in parallel. Lastly, when finding b-correlation questions, we enumerate all the candidate combinations in parallel.}

%\ji{Incremental Techniques: Firstly, The change of local ranking score for the training questions happens only when some tuples in the data changes by transformation rules, so we can recalculate the score by adding or removing the effect of transformed records incrementally. Secondly, the local score of cluster questions are more complicated because that it's related to the matcher, however, we can still get tighter lower bound of cluster size and $Pr(p)$ with program going. Thirdly, we incrementally choose the best transformation group among all possible transform pairs.}


%, different processes exchanged lowest score in top-k every fifty questions.


%We can compute the candidate pairs in parallel. For each candidate pair we can compute its score in parallel. %We computed score of each candidate training rule in parallel, different processes exchanged lowest score in top-k every three questions.


%Each pair in the partition is processed independently in [5]. Thus we can use multiple threads to process the value pairs in parallel, and each value pair will be processed by one thread.


%First, we calculated upper bounds of frequencies of transformation questions and ranked them in parallel. Then, we scanned questions sequentially in each process, and different processes exchanged the highest frequency every twenty questions.


%we enumerate all the candidate question pairs in parallel. For
%according to section \ref{sec:b:x}, then we calculated each group in parallel.
%$(i.ii.i)$ Training Question. First, the coverage of a rule is computed only once, and we do no need to compute the coverage in each round. Second, the utility  ???. Third, we can maintain a score for each training question, and remove the question that has very small score and cannot be selected as a global question. 

%$(i.ii.ii)$ Cluster Question.

%$(i.ii.iii)$ Transformation Question. First, in each step, we only need to compute the top-$k$ questions using pruning techniques and do not need to compute all transformations and then rank them. Second, most of transformation will not be changed in different rounds, and we only need to update the transformations whose records are updated. 


 % Firstly, for ranking a transformation rule, we do not need to enumerate every pair that obeys the rule; instead, we only need to . The change of local ranking score for the training questions happens only when some tuples in the data changes by transformation rules, so we can recalculate the score by adding or removing the effect of transformed records incrementally. Secondly, the local score of cluster questions are more complicated because that it's related to the matcher, however, we can still get tighter lower bound of cluster size and $Pr(p)$ with program going. Thirdly, we incrementally choose the best transformation group among all possible transform pairs 


%we prune records in advance according to the upper bound of score for each rule from updated coverage, accuracy and the upper bound of utility.

%We pruned clusters whose upper bound of score is smaller than current top-k cluster's score. The upper bound of score was calculated from clusters' size and the max utility.
%First, we ranked all the candidate transformation rules according to the upper bound of their frequencies. Second, we calculate the frequency of rules sequentially until we find a rule whose upper bound is smaller than the highest frequency of currently scanned transformation rules.
%$(i.ii)$ Global Ranking.

%$(i.ii.i)$ Training Question. First, the coverage of a rule is computed only once, and we do no need to compute the coverage in each round. Second, the utility  ???. Third, we can maintain a score for each training question, and remove the question that has very small score and cannot be selected as a global question. 

%$(i.ii.ii)$ Cluster Question.  

%$(i.ii.iii)$ Transformation Question. First, in each step, we only need to compute the top-$k$ questions using pruning techniques and do not need to compute all transformations and then rank them. Second, most of transformation will not be changed in different rounds, and we only need to update the transformations whose records are updated.However it is hard to get 100\% accurate rules and we ask human to validate the rules.

s well as several records pairs that satisfy the rule.

The upside is that it is very efficient while the downside is that the correlation among questions is not considered in this case. 


%\hi{Entity Matching Question.} An entity matching question asks the human to verify a record pair and it is the easiest question among the four question types. We can take the cost of an entity matching question as a unit cost.
\begin{equation}
\mathcal{C}(\qt)=\frac{|\qt|}{12}+\frac{11}{12}
\end{equation}
\begin{equation}
\mathcal{C}(\qc)=\frac{|\qc|}{15}+\frac{14}{15}
\end{equation}
\begin{equation}
\mathcal{C}(\qr)=\frac{|\qr|}{3}+\frac{2}{3}
\end{equation}
Since most of the records in the cluster are similar, the cost of a clustering question $\qc$ is larger than 1 and smaller than $|\qc|$, where $|\qc|$ is the number of records in \qt. Intuitively the larger $|\qc|$ is, the larger the cost is. 
Since the records are similar, the cost of a transformation question $\qr$ is larger than 1 and smaller than $|\qr|$, where $|\qr|$ is the number of records associated with \qc. Intuitively the larger $|\qr|$ is, the larger the cost is. 







%We devise a correlation-aware question selection method.

%\add{We might need to give more detailed contributions here.}
%In this paper, we propose a framework to judiciously select questions to maximize the golden-record quality. 
% the cost (human time) and benefit (quality improvement) from asking a question. We then propose an efficient algorithm to .  


%To address the first challenge, we propose a {\it global benefit model} to measure the golden-record quality improvement from asking a question.  %We use the number of changes in the final golden records obtained after asking a question as a way to measure the benefit. 
%As the answer to a question is unknown,  we enumerate all possible answers to a question,  estimate a probability for each answer, and  compute the benefit expectation. 
%We also propose cost models to measure the human time for answering different types of questions (Section~\ref{sec:preliminary}). 
 %As the ground truths of golden records are unknown, we use a small sample of records with ground truths labelled by experts to estimate the benefit. Note that our global benefit model is general and can be used for different types of questions. of answering a question.  We conducted a user study to build  cost models 
%To address the second challenge, we propose to estimate the local benefit for each type of questions based on entropy changes. We then rank the questions and select the top-$k$ best questions for each question type based on the local benefit (Section~\ref{sec:b:1}).  Next, we use the global benefit model to rerank these selected questions, and choose the question with the largest benefit/cost ratio. We also propose a correlation-aware question selection method that considers correlations in selecting high-quality questions (Section~\ref{sec:b:2}).




%In summary, we make the following contributions.








%\subsection{Summary of Experiments}

%\add{added in contribution 4}

%\add{We should add a summary if we have some strong results.}  

%We conducted experiments on three real-world datasets and the 

\iffalse

\subsection{Paper Organization}


We first present the overview of our framework in Section~\ref{sec:preliminary}, and then introduce our benefit model in Section~\ref{sec:b:1}. A correlation-aware method is discussed in Section~\ref{sec:b:2}. We report experimental results in Section~\ref{sec:exp}. We review related work in Section~\ref{sec:rw} and conclude the paper in Section~\ref{sec:con}.

\fi




%For example,  transformation questions are usually generated from clusters and their benefit is usually determined by the cluster size.
%As different questions may require different human effort (or cost) to answer them,  we develop a cost model based on a user study that measures the time it takes to answer each type of question. 
% introduce an iterative estimation-based method  We first obtain a sample of ground-truth for golden records.  Then, for each question (or question combination), we compute the quality improvement (called benefit) using this sample.  Next, we select the question with the largest benefit/cost ratio.  As different questions may require different human effort (or cost) to answer them,  we develop a cost model based on a user study that measures the time it takes to answer each type of question.


\iffalse
% and is a waste of many unnecessary EC operations

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]%\vspace{-1em}
\begin{center}
\centering
\includegraphics[width=\columnwidth]{figs/sequential.pdf}
\vspace{-2em}
\caption{Sequential EM and EC
\label{fig:ex:sequential}}
\end{center}
\vspace{-1.75em}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%


\fi


%validating training rules, validating clusters, and validating transformation rules.  
%%for performing the data integration task 
%entity matching (EM) that generates clusters of duplicate records, data transformation (DT) that transforms variant values into the same format, and entity consolidation (EC) that produces a canonical record for each cluster. % (\aka a {\em golden record}).

%Hence, our problem is to optimize human involvement in a pipeline consisting of entity matching (EM), which generates clusters of duplicate records, and entity consolidation (EC), which generates golden records (GR). These two processes are typically performed consecutively, and point solutions have been studied to improve the quality for either EM~\cite{DBLP:conf/sigmod/ChaiLLDF16,DBLP:conf/sigmod/DasCDNKDARP17,DBLP:conf/sigmod/WangLKFF13} or EC~\cite{DBLP:journals/corr/abs-1709-10436}.

%\vspace{-.5em}

%Traditional algorithms first run EM, followed by EC~\cite{DBLP:journals/corr/abs-1709-10436}, based on the fact that a better EM will find better clusters, thus helping EC. 

%These three phases are typically performed sequentially: (1) asking training rule questions to get some training data, training an entity matching (EM) model~\cite{DBLP:conf/sigmod/ChaiLLDF16,DBLP:conf/sigmod/DasCDNKDARP17,DBLP:conf/sigmod/WangLKFF13} using the training data, finding matching pairs using the EM model and generating clusters based on the matching pairs; (2) asking cluster validation questions to validate the clusters; (3) asking data transformation questions to transform the variant values into the same format~\cite{DBLP:conf/www/HeCCT16,DBLP:conf/sigmod/WangH17,DBLP:conf/sigmod/MorcosAIOPS15,DBLP:journals/pvldb/Singh16,DBLP:conf/icde/AbedjanMIOPS16,DBLP:conf/sigmod/JinACJ17a,DBLP:journals/pvldb/ZhuHC17}; (4) running entity consolidation (EC) algorithms to produce the golden records~\cite{DBLP:journals/corr/abs-1709-10436}.


%each of the three activities above entails domain expertise.  In real world projects, 
%getting the time of domain experts is especially challenging.  Hence  human expertise is  ``the high pole in the tent''.  
%Instead, one needs to optimize human involvement to get the best result within a given human time budget.  
%Alternately, some enterprises want to achieve a specific quality\mourad{Can this be supported? It is hard because we cannot measure the quality without ground truth.}, while minimizing human time.



















%Next we select some questions from \Qall, ask  human to get the results, and generate some training data (for questions in $\mathbb{Q}_T$ and $\mathbb{Q}_C$) and repair the dataset $D$ (for questions in $\mathbb{Q}_R$).  Next we call the machine algorithms using the new training data and the updated  datasets. We repeat the above steps until the budget is used up. Finally we can get the set $G$ of golden records.
%Since these may exist correlation among the questions, it enumerates all permutations of these $b$ questions, runs the machine algorithms to compute the golden records, and evaluates the benefit of each permutation using the samples. 



































\iffalse


\stitle{Holistic Data Integration by Interleaving EM and EC.} Traditional algorithms first run EM and then EC~\cite{DBLP:journals/corr/abs-1709-10436}; a good EM algorithm outputs good clusters making the work of EC easier.
%, based on the fact that a better EM will find better clusters, thus helping EC. 
For example, in Table~\ref{example}, if EM correctly groups the 8 records into 3 correct clusters, 
it will be easier for EC to get correct golden records  on each cluster. 
However, in general EM models can hardly output perfect clusters.
%achieve a perfect 100\% accurate clusters. 
For instance, Figure~\ref{fig:ex:sequential} shows two cases of first running EM then EC. 
In the first case, 
%records \{$r_4,r_5,r_6$\} and records \{$r_7,r_8$\} should belong to two different clusters, but 
EM incorrectly clustered \{$r_4,r_5,r_6$\} and \{$r_7,r_8$\}  together leading EC to not output a golden record for \{$r_7,r_8$\}. 
In the second case, %records \{$r_1,r_2,r_3$\} should be clustered together  but instead 
EC outputted more clusters, \eg
it grouped \{$r_1,r_2$\} in one cluster and $r_3$ in another
since it is hard to match \texttt{EE and CS} with \texttt{Electrical Engineering and Computer Science}. 
Thus, we ended up with three extra golden records.
%the second case will involve 3 duplicated golden records. 
%Evidently, we find that EC can also help EM. 
Looking more carefully at these example, EC and EM could help each other.
For example, starting from the cluster \{$r_4, r_5, r_6$\} as obtained by EM, 
EC will transform \texttt{EE} to \texttt{Electrical Engineering}. 
Similarly, it will transform \textsf{CS} to \textsf{Computer Science} based on \{$r_7, r_8$\}. 
If we then apply these transformations to $r_1$,$r_2$, and $r_3$,
it will be easier for EC to group these records into one cluster.
%Based on these transformations, we can normalize the data, and in this way it is easier to group \{$r_1,r_2,r_3$\} into the same cluster. 
%Thus, EC can make the work of EM easier by normalizing the data. 
%However, existing techniques independently optimize EM and EC.
We thus need a holistic method that interleaves EM and EC to make them benefit each other. 


%\stitle{Human-in-the-loop Data Integration by 
\stitle{Scheduling Human Questions.} Most existing EM and EC methods adopt a human-in-the-loop strategy that utilizes human feedback to improve EM and EC. 
They assume an independent budget for each process, usually in the form of a number of questions to ask human, and 
%that EM and EC have two independent budgets (\ie the number of questions to ask human) and 
schedule the questions independently. 
%In particularly, EM aims to maximize the matching quality and EC focuses on maximizing the golden-record accuracy. 
To interleave EM and EC, a natural question is how to schedule the questions to maximize the accuracy of golden records within a given budget. Moreover EM and EC involve different question types, and  we need to judiciously schedule these questions to optimize EM and EC holistically. 
Next, we use an example to illustrate how to schedule the questions. 




\stitle{Human Questions}.  We consider three types of questions and our techniques can be easily extended for other types.
%to support  any EM and EC questions. 
{\it (1) Training Rule Questions.} Machine-learning-based EM\footnote{We focus on ML methods which usually delivers state-of-the-art results for EM.}~\cite{GokhaleDDNRSZ14,DBLP:journals/pvldb/KondaDCDABLPZNP16} needs training data, \ie matching/non-matching pairs, to train a model. %, \eg random forest. 
They usually utilize training rules to get training data~\cite{DBLP:journals/vldb/WhangG14};
%where each training rule is a 
these rules are in the form of ``if-condition-then-matching (non-matching)'', \eg if the Jaccard similarity of two addresses is larger than 0.5, then the two records should refer to the same entity. 
If a rule is approved, then the record pairs that satisfy the rule are used as a training data.
% data to enhance the EM model.   
%
{\it (2) Clustering Question.}  
A human is asked to validate a cluster of records.
%To check whether the records in a cluster refer to the same entity, we can ask a human to validate a cluster of records. 
If the records  do not refer to the same entity, the cluster is split into sub-clusters where all records in each sub-cluster refer to the same entity. 
Note that training rule questions aim to 
cluster together records referring to the same entity 
%merge records referring to the same entity into the same cluster 
while clustering questions split clusters that do not refer to the same entity into sub-clusters. They thus complement each other to achieve higher clustering quality. 
%
{\it (3) Transformation Rule Questions.} 
A common approach for EC is to use a master data management system based on human-written rules~\ref{}.
However, such an approach does not scale with the data as the number of rules could be in the thousands.
In this paper, we consider approaches (\eg~\cite{DBLP:journals/corr/abs-1709-10436}) that generate 
transformation rules from the data itself to perform the consolidation, \eg  \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering}.  
%As different records may have different representations for the same entity, 
%some methods~\cite{DBLP:journals/corr/abs-1709-10436} use transformation rules to transform the data to the same format, \eg  \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering}.  
In this case, we ask a human to validate a transformation rule, $v\rightarrow v'$, to check whether the value $v$ should be transformed/repaired to another value $v'$ for the records containing value $v$, 
\eg \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering} in $r_3$. 
If the rule is approved, we use the rule to transform the data. 

%As different records may have different representations for the same entity, 
%some methods~\cite{DBLP:journals/corr/abs-1709-10436} use transformation rules to transform the data to the same format, \eg  \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering}.  
%We can ask a human to validate a transformation question, where each question $v\rightarrow v'$ asks a human to check whether the value $v$ should be repaired to another value $v'$ for the records containing value $v$, 
%\eg  \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering} in $r_3$. 
%If the transformation rule is approved, we transform the data using this rule. %the transformation rule.  

Figure~\ref{fig:ex:1} shows an example that interleaves EM and EC. % by scheduling the questions. 
We first ask a training rule question, ``if the Zipcode values are the same, then the records match'',
which is used to obtain labeled data to train a model that would then generate three clusters. 
\mourad{the training rule questions are used to generate training data which in turn is used to train an EM model, that model is then used to get clusters. Right? YES}
We then ask a cluster question for $\{r_4,r_5,r_6,r_7,r_8\}$), which leads to splitting the cluster into two sub-clusters $\{r_4,r_5,r_6\}$ and $\{r_7,r_8\}$. 
Next, we ask a transformation question, \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering}, based on the cluster $\{r_4,r_5,r_6\}$. As the transformation is approved, $r_3$ is modified by changing \texttt{EE} to \texttt{Electrical Engineering}. 
%Based on the normalized data, 
Subsequently, the EM model is updated and 
 the \texttt{Name} attribute will play an important role to find matching pairs\mourad{What do you mean by ``uses the \texttt{Name}  attribute'' Update} which leads to merging $r_1,r_2$, and $r_3$ as one cluster. 
This creates an opportunity for a new transformation, namely \texttt{CS} $\rightarrow$ \texttt{Computer Science}.
At the end, we replace  \texttt{02141} by \texttt{02142} in the Zipcode attribute using majority voting 
and obtain the correct golden records.
%Then it transforms \texttt{CS} to  \texttt{Computer Science}, \texttt{02141} to \texttt{02142}\mourad{Why?}, and finally we can get the correct golden records.

\fi


%Figure~\ref{fig:ex:1} shows an example that interleaves EM and EC by scheduling the above types of questions. 
%It first asks a training rule question (if the Zipcode values are the same, then the records match) to get three clusters. 
%\mourad{I'm confused here, the training rule questions are used to generate training data which in turn is used to train an EM model, that model is then used to get clusters. But here you're skipping all of this?}
%Then it asks a cluster question (cluster $\{r_4,r_5,r_6,r_7,r_8\}$) and splits the cluster into two sub-clusters $\{r_4,r_5,r_6\}$ and $\{r_7,r_8\}$. 
%Next it asks a transformation question (\texttt{EE} $\rightarrow$ \texttt{Electrical Engineering}) based on the cluster $\{r_4,r_5,r_6\}$. As the question is approved, it normalizes record $r_3$ by transforming \texttt{EE} to \texttt{Electrical Engineering}. Based on the normalized data, the EM model will be updated and it uses the \texttt{Name} attribute to find matching pairs which can merge $r_1,r_2,r_3$ as a cluster. Then it transforms \texttt{CS} to  \texttt{Computer Science}, \texttt{02141} to \texttt{02142}, and finally we can get the correct golden records.
%>>>>>>> c367344c438030bbc926e973c0da9800ba7da81b





 


















%For example, if the clusters have low quality, we want to ask more EM questions to improve the clustering quality; while if the clusters already have high precision, we want to ask more EC questions to get the canonical or preferred values for each attribute. 


%they cannot use EC to help EM. because EM and EC help each other

%They will ask different types of questions to get human feedback. However they independently asks the questions and do not schedule the questions holistically. Next we take 3 types of questions as examples. 

%  For example, for training rule questions, the rules with  large accuracy and coverage have large benefit to enhance the EM model. For transformation rule questions, the rules that can be applied to many records have large benefit to normalize the data.  Note that  and , thus it is rather challenging  to quantify the benefit for each question. 
%effective techniques to select questions for maximizing the golden-record quality.  
%training rule questions and clustering question can improve the cluster quality, while the transformation questions can normalize the data.

%For example, to get high-quality clusters, EM will ask human to validate a rule, e.g., if two records have larger similarity on the \texttt{Name} attribute, then the two records refer to the same entity.  

%There are three question types, training questions, clustering questions and transformation questions if running EM and EC holistically\footnote{Our method can support any other types of questions, e.g, asking a pair of records whether they refer to the same entity.}.  
%%\begin{example}
%\add{We should move this example to latter sections. Here, we can just list questions and say there are different ways of scheduling, but discuss what and how later.}
%\end{example}


%\mourad{Not sure we actually need this third observation.}
%\stitle{3. Saving operations to be goal (golden record)-oriented.} A user usually has a budget and aims to maximize the accuracy of golden record. Thus we need to avoid unnecessary human involvement and take full use of the budget to enhance the accuracy of golden records. For example, if most records have the same value on an attribute, we can use majority voting to get the canonical value and avoid asking more questions.







%\hi{Entity Matching.} We take machine-learning-based EM as an example. It requires to provide some training data (e.g., matching/non-matching pairs) and use them to train an EM matching model (e.g., random forest). Next it uses the EM model to check each record pair and return a set of candidate matching pairs \footnote{For large datasets, it is prohibitively expensive to provide all pairs to the EM tool, and it usually first uses some blocking rules to prune the pairs that have low possibility to be matching and feeds the non-matching pairs to the EM tool.}. Finally, it groups the candidate matching pairs into some clusters, such that  the two records in the same matching pair will be in the same cluster.  Note that it is expensive to provide much training data. To address this problem, training rules can be used, where each training rule is a ``if-condition-then-matching (non-matching)'', \eg rule $\phi_1$: if the Jaccard similarity of two addresses is larger than 0.5, then the two records refer to the same entity. We can ask human to validate the rules, and if the rules are approved, then the record pairs that satisfy the rules can be taken as the training data. To further improve the EM model, we can also ask human to validate a cluster of records. If the records in the cluster do not refer to the same entity, the cluster will be to split into sub-clusters where all records in each sub-cluster refer to the same entity. Based on the answers of cluster questions, we can get some validated matching pairs that are in the same cluster and some validated non-matching pairs that are from different sub-clusters. Then we can feed theses pairs to the EM tool. 

%\hi{Entity Consolidation.} A straightforward uses a majority-voting algorithm to vote the golden value for each cluster. Since different records may have different representations on the same entity, some methods~\cite{DBLP:journals/corr/abs-1709-10436} use transformation rules to transform the data to the same format, e.g., \#th $\rightarrow$ \# (e.g., transferring 50th to 50).  We can ask human to validate a transformation question, where each question $v\rightarrow v'$ asks human to check whether the value $v$ should be repaired to another value $v'$ for the records containing value $v$ (e.g., transferring 50th to 50 in records $r_3,r_4$ and 32nd to 32 in records $r_5,r_7$). If the question is approved by human, we transform the data using the transformation rule.

% quality by asking training rule questions and cluster questions 


%by asking transformation questions.
%\stitle{Separating EM and EC.}  In this paper, we find that EM and EC can benefit each other and we propose a framework for holistic data integration by interleaving EM and EC.

%\begin{example}
%[Separating EM and EC]
%\nan{We should add an example to show the case if we do EM and EC consecutively.}
%\end{example}


%\stitle{Key Observations.} Looking at the two data integration processes, we make the following observations.

%\mourad{Would it possible to show these through an example?}:

\fi








\iffalse


\stitle{Holistic Data Integration by Interleaving EM and EC.} Traditional algorithms first run EM and then EC~\cite{DBLP:journals/corr/abs-1709-10436}; a good EM algorithm outputs good clusters making the work of EC easier.
%, based on the fact that a better EM will find better clusters, thus helping EC. 
For example, in Table~\ref{example}, if EM correctly groups the 8 records into 3 correct clusters, 
it will be easier for EC to get correct golden records  on each cluster. 
However, in general EM models can hardly output perfect clusters.
%achieve a perfect 100\% accurate clusters. 
For instance, Figure~\ref{fig:ex:sequential} shows two cases of first running EM then EC. 
In the first case, 
%records \{$r_4,r_5,r_6$\} and records \{$r_7,r_8$\} should belong to two different clusters, but 
EM incorrectly clustered \{$r_4,r_5,r_6$\} and \{$r_7,r_8$\}  together leading EC to not output a golden record for \{$r_7,r_8$\}. 
In the second case, %records \{$r_1,r_2,r_3$\} should be clustered together  but instead 
EC outputted more clusters, \eg
it grouped \{$r_1,r_2$\} in one cluster and $r_3$ in another
since it is hard to match \texttt{EE and CS} with \texttt{Electrical Engineering and Computer Science}. 
Thus, we ended up with three extra golden records.
%the second case will involve 3 duplicated golden records. 
%Evidently, we find that EC can also help EM. 
Looking more carefully at these example, EC and EM could help each other.
For example, starting from the cluster \{$r_4, r_5, r_6$\} as obtained by EM, 
EC will transform \texttt{EE} to \texttt{Electrical Engineering}. 
Similarly, it will transform \textsf{CS} to \textsf{Computer Science} based on \{$r_7, r_8$\}. 
If we then apply these transformations to $r_1$,$r_2$, and $r_3$,
it will be easier for EC to group these records into one cluster.
%Based on these transformations, we can normalize the data, and in this way it is easier to group \{$r_1,r_2,r_3$\} into the same cluster. 
%Thus, EC can make the work of EM easier by normalizing the data. 
%However, existing techniques independently optimize EM and EC.
We thus need a holistic method that interleaves EM and EC to make them benefit each other. 


%\stitle{Human-in-the-loop Data Integration by 
\stitle{Scheduling Human Questions.} Most existing EM and EC methods adopt a human-in-the-loop strategy that utilizes human feedback to improve EM and EC. 
They assume an independent budget for each process, usually in the form of a number of questions to ask human, and 
%that EM and EC have two independent budgets (\ie the number of questions to ask human) and 
schedule the questions independently. 
%In particularly, EM aims to maximize the matching quality and EC focuses on maximizing the golden-record accuracy. 
To interleave EM and EC, a natural question is how to schedule the questions to maximize the accuracy of golden records within a given budget. Moreover EM and EC involve different question types, and  we need to judiciously schedule these questions to optimize EM and EC holistically. 
Next, we use an example to illustrate how to schedule the questions. 




\stitle{Human Questions}.  We consider three types of questions and our techniques can be easily extended for other types.
%to support  any EM and EC questions. 
{\it (1) Training Rule Questions.} Machine-learning-based EM\footnote{We focus on ML methods which usually delivers state-of-the-art results for EM.}~\cite{GokhaleDDNRSZ14,DBLP:journals/pvldb/KondaDCDABLPZNP16} needs training data, \ie matching/non-matching pairs, to train a model. %, \eg random forest. 
They usually utilize training rules to get training data~\cite{DBLP:journals/vldb/WhangG14};
%where each training rule is a 
these rules are in the form of ``if-condition-then-matching (non-matching)'', \eg if the Jaccard similarity of two addresses is larger than 0.5, then the two records should refer to the same entity. 
If a rule is approved, then the record pairs that satisfy the rule are used as a training data.
% data to enhance the EM model.   
%
{\it (2) Clustering Question.}  
A human is asked to validate a cluster of records.
%To check whether the records in a cluster refer to the same entity, we can ask a human to validate a cluster of records. 
If the records  do not refer to the same entity, the cluster is split into sub-clusters where all records in each sub-cluster refer to the same entity. 
Note that training rule questions aim to 
cluster together records referring to the same entity 
%merge records referring to the same entity into the same cluster 
while clustering questions split clusters that do not refer to the same entity into sub-clusters. They thus complement each other to achieve higher clustering quality. 
%
{\it (3) Transformation Rule Questions.} 
A common approach for EC is to use a master data management system based on human-written rules~\ref{}.
However, such an approach does not scale with the data as the number of rules could be in the thousands.
In this paper, we consider approaches (\eg~\cite{DBLP:journals/corr/abs-1709-10436}) that generate 
transformation rules from the data itself to perform the consolidation, \eg  \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering}.  
%As different records may have different representations for the same entity, 
%some methods~\cite{DBLP:journals/corr/abs-1709-10436} use transformation rules to transform the data to the same format, \eg  \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering}.  
In this case, we ask a human to validate a transformation rule, $v\rightarrow v'$, to check whether the value $v$ should be transformed/repaired to another value $v'$ for the records containing value $v$, 
\eg \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering} in $r_3$. 
If the rule is approved, we use the rule to transform the data. 

%As different records may have different representations for the same entity, 
%some methods~\cite{DBLP:journals/corr/abs-1709-10436} use transformation rules to transform the data to the same format, \eg  \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering}.  
%We can ask a human to validate a transformation question, where each question $v\rightarrow v'$ asks a human to check whether the value $v$ should be repaired to another value $v'$ for the records containing value $v$, 
%\eg  \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering} in $r_3$. 
%If the transformation rule is approved, we transform the data using this rule. %the transformation rule.  

Figure~\ref{fig:ex:1} shows an example that interleaves EM and EC. % by scheduling the questions. 
We first ask a training rule question, ``if the Zipcode values are the same, then the records match'',
which is used to obtain labeled data to train a model that would then generate three clusters. 
\mourad{the training rule questions are used to generate training data which in turn is used to train an EM model, that model is then used to get clusters. Right? YES}
We then ask a cluster question for $\{r_4,r_5,r_6,r_7,r_8\}$), which leads to splitting the cluster into two sub-clusters $\{r_4,r_5,r_6\}$ and $\{r_7,r_8\}$. 
Next, we ask a transformation question, \texttt{EE} $\rightarrow$ \texttt{Electrical Engineering}, based on the cluster $\{r_4,r_5,r_6\}$. As the transformation is approved, $r_3$ is modified by changing \texttt{EE} to \texttt{Electrical Engineering}. 
%Based on the normalized data, 
Subsequently, the EM model is updated and 
 the \texttt{Name} attribute will play an important role to find matching pairs\mourad{What do you mean by ``uses the \texttt{Name}  attribute'' Update} which leads to merging $r_1,r_2$, and $r_3$ as one cluster. 
This creates an opportunity for a new transformation, namely \texttt{CS} $\rightarrow$ \texttt{Computer Science}.
At the end, we replace  \texttt{02141} by \texttt{02142} in the Zipcode attribute using majority voting 
and obtain the correct golden records.
%Then it transforms \texttt{CS} to  \texttt{Computer Science}, \texttt{02141} to \texttt{02142}\mourad{Why?}, and finally we can get the correct golden records.

\fi


%Figure~\ref{fig:ex:1} shows an example that interleaves EM and EC by scheduling the above types of questions. 
%It first asks a training rule question (if the Zipcode values are the same, then the records match) to get three clusters. 
%\mourad{I'm confused here, the training rule questions are used to generate training data which in turn is used to train an EM model, that model is then used to get clusters. But here you're skipping all of this?}
%Then it asks a cluster question (cluster $\{r_4,r_5,r_6,r_7,r_8\}$) and splits the cluster into two sub-clusters $\{r_4,r_5,r_6\}$ and $\{r_7,r_8\}$. 
%Next it asks a transformation question (\texttt{EE} $\rightarrow$ \texttt{Electrical Engineering}) based on the cluster $\{r_4,r_5,r_6\}$. As the question is approved, it normalizes record $r_3$ by transforming \texttt{EE} to \texttt{Electrical Engineering}. Based on the normalized data, the EM model will be updated and it uses the \texttt{Name} attribute to find matching pairs which can merge $r_1,r_2,r_3$ as a cluster. Then it transforms \texttt{CS} to  \texttt{Computer Science}, \texttt{02141} to \texttt{02142}, and finally we can get the correct golden records.
%>>>>>>> c367344c438030bbc926e973c0da9800ba7da81b





 


















%For example, if the clusters have low quality, we want to ask more EM questions to improve the clustering quality; while if the clusters already have high precision, we want to ask more EC questions to get the canonical or preferred values for each attribute. 


%they cannot use EC to help EM. because EM and EC help each other

%They will ask different types of questions to get human feedback. However they independently asks the questions and do not schedule the questions holistically. Next we take 3 types of questions as examples. 

%  For example, for training rule questions, the rules with  large accuracy and coverage have large benefit to enhance the EM model. For transformation rule questions, the rules that can be applied to many records have large benefit to normalize the data.  Note that  and , thus it is rather challenging  to quantify the benefit for each question. 
%effective techniques to select questions for maximizing the golden-record quality.  
%training rule questions and clustering question can improve the cluster quality, while the transformation questions can normalize the data.

%For example, to get high-quality clusters, EM will ask human to validate a rule, e.g., if two records have larger similarity on the \texttt{Name} attribute, then the two records refer to the same entity.  

%There are three question types, training questions, clustering questions and transformation questions if running EM and EC holistically\footnote{Our method can support any other types of questions, e.g, asking a pair of records whether they refer to the same entity.}.  
%%\begin{example}
%\add{We should move this example to latter sections. Here, we can just list questions and say there are different ways of scheduling, but discuss what and how later.}
%\end{example}


%\mourad{Not sure we actually need this third observation.}
%\stitle{3. Saving operations to be goal (golden record)-oriented.} A user usually has a budget and aims to maximize the accuracy of golden record. Thus we need to avoid unnecessary human involvement and take full use of the budget to enhance the accuracy of golden records. For example, if most records have the same value on an attribute, we can use majority voting to get the canonical value and avoid asking more questions.







%\hi{Entity Matching.} We take machine-learning-based EM as an example. It requires to provide some training data (e.g., matching/non-matching pairs) and use them to train an EM matching model (e.g., random forest). Next it uses the EM model to check each record pair and return a set of candidate matching pairs \footnote{For large datasets, it is prohibitively expensive to provide all pairs to the EM tool, and it usually first uses some blocking rules to prune the pairs that have low possibility to be matching and feeds the non-matching pairs to the EM tool.}. Finally, it groups the candidate matching pairs into some clusters, such that  the two records in the same matching pair will be in the same cluster.  Note that it is expensive to provide much training data. To address this problem, training rules can be used, where each training rule is a ``if-condition-then-matching (non-matching)'', \eg rule $\phi_1$: if the Jaccard similarity of two addresses is larger than 0.5, then the two records refer to the same entity. We can ask human to validate the rules, and if the rules are approved, then the record pairs that satisfy the rules can be taken as the training data. To further improve the EM model, we can also ask human to validate a cluster of records. If the records in the cluster do not refer to the same entity, the cluster will be to split into sub-clusters where all records in each sub-cluster refer to the same entity. Based on the answers of cluster questions, we can get some validated matching pairs that are in the same cluster and some validated non-matching pairs that are from different sub-clusters. Then we can feed theses pairs to the EM tool. 

%\hi{Entity Consolidation.} A straightforward uses a majority-voting algorithm to vote the golden value for each cluster. Since different records may have different representations on the same entity, some methods~\cite{DBLP:journals/corr/abs-1709-10436} use transformation rules to transform the data to the same format, e.g., \#th $\rightarrow$ \# (e.g., transferring 50th to 50).  We can ask human to validate a transformation question, where each question $v\rightarrow v'$ asks human to check whether the value $v$ should be repaired to another value $v'$ for the records containing value $v$ (e.g., transferring 50th to 50 in records $r_3,r_4$ and 32nd to 32 in records $r_5,r_7$). If the question is approved by human, we transform the data using the transformation rule.

% quality by asking training rule questions and cluster questions 


%by asking transformation questions.
%\stitle{Separating EM and EC.}  In this paper, we find that EM and EC can benefit each other and we propose a framework for holistic data integration by interleaving EM and EC.

%\begin{example}
%[Separating EM and EC]
%\nan{We should add an example to show the case if we do EM and EC consecutively.}
%\end{example}


%\stitle{Key Observations.} Looking at the two data integration processes, we make the following observations.

%\mourad{Would it possible to show these through an example?}:













\iffalse
% !TEX root = main.tex
\section{Introduction}
\label{sec:introduction}


Having examined about 100 real world data integration projects, executed by the data integration company, Tamr\footnote{https://www.tamr.com}, we have seen a common theme to almost all of them. Specifically:


a) Projects entail obtaining training data to construct a machine learning (ML) deduplication module, followed by execution of the deduplication code to construct clusters of like records. Lastly, the clusters must be reduced to a golden record for each cluster, which is the final output.

b)	Projects must be executed at scale, i.e. for millions of records.  For example, Toyoto Motor Europe is integrating approximately 30M customer records from 250 data bases around the continent in 40 different languages.  Other projects exhibit similar scale. Executing at scale requires careful optimization of the integration pipeline, but even more careful optimization of human involvement.

c)	Human involvement entails three activities.  First, it is hopeless at scale to generate training data one pair of records at a time.  Instead, training data is inevitably constructed from a collection of human-written rules.  One such rules might be ``{\it if the Jaccard similarity of the addresses of two companies is larger than 0.8, then the two companies represent the same entity}''. Hence, a human must check the validity of such human written rules.  Then, running an ML codeline using the training data will produce clusters of allegedly duplicate records.  Clusters must be checked by a human to ascertain model validity.  Lastly, a rule-driven golden record system must be run to reduce each cluster to a single golden record, which is the final outcome. 

d) At scale, human involvement must be optimized, since each of the three activities above entails domain expertise.  In real world projects, getting the time of domain experts is especially challenging.  Hence human expertise is  ``the high pole in the tent''.  There is no hope of exhaustively checking all three steps above.  Instead, one needs to optimize human involvement to get the best result possible within a given human time budget.  Alternately, some enterprises want to achieve a specific quality, while minimizing human time.

\input{example_table}


Hence, our problem is to optimize human involvement in a pipeline consisting of entity matching (EM), which generates clusters of duplicate records, and entity consolidation (EC), which generates golden records (GR). These two processes are typically performed consecutively, and point solutions have been studied to improve the quality for either entity matching ~\cite{DBLP:conf/sigmod/ChaiLLDF16,DBLP:conf/sigmod/DasCDNKDARP17,DBLP:conf/sigmod/WangLKFF13} or entity consolidation~\cite{DBLP:journals/corr/abs-1709-10436}.


Traditional algorithms first run EM and then EC~\cite{DBLP:journals/corr/abs-1709-10436}, based on the fact that a better EM will find better clusters, thus helping EC. For example, In Table~\ref{example}, if EM can group the 8 records into 3 correct clusters, EC can get correct golden records for each cluster.  However, in practice, EM models never achieve 100\% accuracy, because there is never enough accurate training data .  For instance, Figure~\ref{fig:ex:sequential} shows two cases that first run EM and then EC.  In the first case, records \{$r_4,r_5,r_6$\} and records \{$r_7,r_8$\}   belong to two different clusters, but EM incorrectly clusters them together. Therefore EC will miss the golden record for \{$r_7,r_8$\}. 
In the second case, records \{$r_1,r_2,r_3$\} are incorrectly grouped into two clusters  \{$r_1,r_2$\} and $\{r_3\}$,  because it is hard to match \texttt{EE and CS} with \texttt{Electrical Engineering and Computer Science}. Thus, the second case will involve 3 duplicated golden records.  

Note clearly that EC can also help EM. For example, based on the cluster \{$r_4, r_5, r_6$\},  EC will transform \texttt{EE} to \texttt{Electrical Engineering}. Similarly, EC will transform \textsf{CS} to \textsf{Computer Science} based on the cluster of \{$r_7, r_8$\}. Based on these transformations, it is easier to group \{$r_1,r_2,r_3$\} into the same cluster.  Thus, EC can make the work of EM easier by normalizing the data.  


As a result, existing techniques that optimize EM and EC, by allocating a human budget to each one independently, are clearly flawed.  Therefore, we need a holistic method that iteratively interleaves EM and EC for mutual benefit.


\stitle{Challenges.} Two key challenges need to be addressed to holistically schedule human input: 

\hi{(1) How to quantify the questions?} Different questions have different benefit to  golden record quality and it is hard to quantify the ``benefit'' of each question, because 
$(i)$~we do not know the answer to each question before we ask it 
and $(ii)$~we have no ground-truth for  golden records to compute the improvement from asking a question. Moreover, EM and EC questions are not comparable because they have different optimization goals. In addition, different questions take different amounts of human time (e.g., a cluster validation question for a large cluster will take more human time than that for a small one). Hence we need to rank the questions by considering both their benefit and time cost. 


\hi{(2) How to select ``high-quality'' questions?}  There are a large number of possible questions, and it is expensive to enumerate every question and select the best one.  Moreover, questions may be correlated to each other. For example,  transformation questions are usually generated from clusters and their benefit is usually determined by the cluster size. It is prohibitively expensive to enumerate a combination of multiple questions. 


In this paper, we introduce an iterative estimation-based method to  judiciously select questions to maximize the golden-record quality.  
We first obtain a sample of  ground-truth golden records.  Then, for each question (or question combination), we compute the quality improvement (called benefit) using this sample.  Next, we select the question with the largest benefit/cost ratio.  As different questions may require different human effort (or cost) to answer them,  we develop a cost model based on a user study that measures the time it takes to answer each type of question.


\stitle{Contributions.}  We make the following contributions.

\noindent (1)  We propose a human-in-the-loop holistic data integration framework that interleaves EM and EC to improve the quality of data integration.


\noindent (2)  We develop a question scheduling framework that judiciously selects the questions within a human time budget to maximize the accuracy of golden records.


\noindent (3) We propose effective techniques to quantify the benefit and cost of different questions.

\noindent (4) We perform extensive experiments on three real-world datasets and show that our method significantly outperforms existing solutions. 














%  it aims to select the best question sequence among these $b$ questions by enumerating all permutations, and it adopts the permutation with the largest benefit, and recomputes \Qc, \Qr and \Qt.           

%computed by two strategies. The first is using the samples $S$ to estimate the accuracy of %is to find more record pairs that cannot be discriminated by the EM model.  We want to first ask the rule that contain more pairs that are hard to be discriminated by the EM model.
%Then we can use the sum of the uncertainty of these pairs to sort the rules, i.e, %we can get a set $\qc \times \qc$ of pairs by enumerating every record pair.  We
%select the next questions from the question types with the same as the two best questions. Iteratively this method can utilize the two dimension correlations to select questions.
%For example, if $Q_x$ is \qt, then we select the  best question from \Qt.  

%In this way, we can get the question sequence with the largest benefit improvement.

%Note that this method requires to enumerate every two questions and it is expensive to run the machine algorithms $\mathcal{O}(N^2)$ times for $N$ question types. To address this issue, we have an observation that we can easily detect some questions have no correlations. For example, considering a training rule question and a cluster question. If they have large overlap on their records, they have negative correlation. In this case, we do not need to enumerate such question pairs. On the other hand, the entity matching question (training rule question, clustering question) may have positive  correlation with the data repairing question if one of them cannot improve the golden-record precision while they together can improve the golden-record precision. In this way, we can avoid enumerating the unnecessary question pairs and reduce the complexity of calling the machine algorithms. 


% it is very efficient to select a question, but it has two limitations. First, it does not consider the correlations between questions.  Second, it i
%In addition, we can also select multiple questions (e.g., selecting $b$ questions in each round) in each time to reduce the number of calls to the machine algorithms.
%Consider clustering questions and entity matching questions. They will generate more training data and have no positive correlation. Instead, they may have negative correlation. For example, if a clustering question covers an entity matching question (i.e., the cluster contains the two records of the entity pair), then they have negative correlation. Similarly, if 

%computed by two strategies. The first is using the samples $S$ to estimate the accuracy of 
%is to find more record pairs that cannot be discriminated by the EM model.  We want to first ask the rule that contain more pairs that are hard to be discriminated by the EM model.
%Then we can use the sum of the uncertainty of these pairs to sort the rules, i.e, 



%In this section, we first assume that each question has the same cost, e.g., a training rule question, a clustering question and a transformation question takes the same human time to answer the question. We will discuss how to support the case that different questions have different costs in Section~\ref{sec:cost}. 


%and we find that the cost follows the linear model and get the following cost functions. 
%\begin{equation}
%\mathcal{C}=\alpha |Q|+\beta
%\end{equation}
%\noindent where $\mathcal{C}$ is the cost of a question $Q$, $\alpha$ and $\beta$ are two parameters.  For different question types, we only need to instantiate the two parameters. 


%The machine algorithm usually cannot produce high-quality golden records, because the data is rather dirty and it requires to involve human to improve the quality.  For example, it is hard to cluster $r_1,r_2,r_3$ together without normalizing the data.

%\hi{Human-in-the-loop Method.} We propose a human-in-the-loop data integration framework that judiciously schedules the questions and calls the machine algorithm based on the answers of these questions. Figure~\ref{fig:arch1} shows the workflow of our system.

%Initially, we generate three question sets \Qt, \Qc, and \Qr based on the machine algorithms. Toward this goal, Then we run the machine algorithms to generate the clusters and infer the golden records. In this way, 

%For each question, we get more training data to enhance the EM model or update the dataset $D$. Specifically
%$\mathbb{Q}_T$, if the rule is approved, we take the record pairs that satisfy the rule as training data. For a clustering question \Qc,  if the records in the cluster refer to the same entity, each pair is taken as a matching pair; if the records are split into several sub-clusters, then the records in the same sub-cluster are taken as matching pairs and the records from different sub-clusters are taken as non-matching pairs. These matching or non-matching pairs are taken as training data. For a transformation rule question \Qr, we update the dataset $D$. 
%Given a budget to ask human, we aim to select a sequence of questions $\Qs=\langle Q_1,Q_2, \cdots, Q_B\rangle$ to ask human in order to maximize  the accuracy of golden records, where $Q_i$ is either a training rule question, clustering question or transformation question.  $B$ questions to maximize the accuracy of the golden records,  %where the accuracy is the percentage of correct golden records.  



%For example, for the $i$-th attribute, it selects the majority value in this attribute as the golden attribute value. Then the golden record is composed of the golden values on each attribute in the cluster. 
% %For each cluster $C\in \mathbb{C}$, it aims to generate a golden record $G$. Assume there are $x$ records $r_1,r_2,\cdots, r_x$ in the cluster. 


%\begin{definition} \textsc{(Holistic Data Integration)} 
%\end{definition}


%maximize the accuracy of obtained golden records (GR) with a human-cost budget.

%Entity matching is used to generate the clusters and entity consolidation is used to infer the golden values for each cluster. 

%\nan{We should add (simplified) definitions of questions here. Also we need to define the input/output of EM and EC. Otherwise, we cannot define the studied problem -- it should be the optimization problem of minimizing the number of questions, instead of the golden record problem.}
%, which judiciously selects questions to ask human, calls the machine modules based on the human answers of these questions, and computes the golden records. 
% \mourad{This is a bit confusing; Are we we assuming that there is a machine-only pipeline, which starts from the input data and output the golden records with no human involvement? But this is not possible, EM needs some training data or an expert providing rules; MV doesn't work if it's the only thing we do in EC, we need humans.}  (e.g., random forest) by providing some training data (e.g., matching/non-matching pairs). Then it utilizes blocking rules to prune the  pairs that have low possibility to be matching. Next 
%the the record of a golden record is the entity consolidation aims to generate a table $G$ with $g$ golden records, such that, 
\iffalse
\be
	\item {\bf No duplicate:} Any two records $r_1, r_2$ in $G$ do not refer to the same entity. 

	\item {\bf Correct golden attribute value:} For each record $r$ in $G$, its attribute value is a canonical value. 

	\item {\bf Complete:} For any record $r$ in $D$, there exists a record $r'$ in $G$ which refers to the same entity with $r$.
\ee
\vspace*{-4ex}
\fi
%Given a set of training rule questions \Qt,  a set of clustering questions \Qc, and a set of transformation questions \Qr,  and 
%For each question, it asks human to get the answers, runs the machine algorithms, and asks the next questions. Iteratively, it can get the golden records. 

%Initially, we need to run the machine algorithms to generate question sets \Qt, \Qc, and \Qr. Toward this goal, we require to get some training data to train the EM model. We select several training rules to get such training data (we will discuss the details on how to select training rule questions in Section~\ref{subsec:sorting}). Then we run the machine algorithms to generate the clusters and infer the golden records. In this way, we can generate three sets of questions, $\mathbb{Q}_T$, $\mathbb{Q}_C$, and  $\mathbb{Q}_R$.  

%\subsection{System Overview} 

% It first runs the machine algorithm to generate some questions. Then it judiciously selects questions to ask human, calls the machine algorithm based on the human answers of these questions, and computes the golden records. 






%Suppose we have three sets of questions, training rule questions $\Qt$, clustering questions $\Qc$, and transformation questions \Qr. (We will formulate define the questions and discuss how to generate the questions in Section~\ref{subsec:human}). Let $\Qall = \Qt\cup \Qc\cup \Qr$ denote the set of all possible questions. 



% and $\mathbb{Q}_C$, we get some training data. and generates some training data () and repairs the dataset $D$ (for questions in $\mathbb{Q}_R$).  Next it calls the machine modules using the new training data and the updated datasets. It repeats the above steps until the budget is used up. 


%\hi{Question Scheduler.}  
Intuitively, the cost of a question depends on the time used to answer a question. To this end, w



% in the cluster of $\{r_1, r_2, r_3, r_7,r_8\}$, the data is rather dirty and the voting based method cannot obtain the golden value without data normalization/repair, e.g,. street $\rightarrow$ st, and 50th $\rightarrow$ 50. 

%Thus we want to generates some questions, e.g., training rule set $\mathbb{Q}_T$, clustering question set $\mathbb{Q}_C$, and transformation question set $\mathbb{Q}_R$, we want to utilize human feedback on some of these questions to improve the quality of golden records.




%

% of records. 
%If the records in the cluster do not refer to the same entity, human is required to split the records in the cluster into several sub-clusters where all records in each sub-cluster refer to the same entity; otherwise, all the records in the cluster are validated to be matching.
%A rule $v\rightarrow v'$ repairs all the records with value $v$ to the value $v'$. We can ask human to validate the rule. If the rule is approved, we use the rule to transform the data; otherwise we skip the rule.  
 repairing rule can be applied to the records.

 as well as a sample of records with value $v$. 

Given a set of tables with lined up attributes\footnote{We assume that schema matching has been performed.}, 
integrating them typically involve two processes:
entity matching (EM), \ie finding clusters of records that represent the same entity,  
and entity consolidation (EC), \ie merging each cluster into a ``golden record'' containing the canonical or preferred values for each attribute. 
%EM aims to generate high-quality clusters while EC emphasizes on inferring the golden records from each cluster. 
These two processes are typically performed consecutively, and point solutions have been studied to improve the quality for either entity matching~\cite{DBLP:conf/sigmod/ChaiLLDF16,DBLP:conf/sigmod/DasCDNKDARP17,DBLP:conf/sigmod/WangLKFF13}, or entity consolidation~\cite{DBLP:journals/corr/abs-1709-10436}.
However, there is not solution that tackles these two processes in a unified manner. 


%The duplicates are typically described as the records that re- fer to the same real-world objects. Handling duplicates, i.e., detecting (a.k.a. entity resolution or record linkage) and re- moving (a.k.a. entity consolidation) them, is a key aspect of data quality and data integration.

%Two key processes in data integration are entity matching (EM), \ie finding clusters of records that represent the same entity,  and entity consolidation (EC), \ie merging each cluster into a ``golden record'' which contains the canonical or preferred values for each attribute.  In practice, these processes are typically performed consecutively,  first EM, then EC. Moreover, each process heavily depends on human expertise, e.g., asking human to validate training rules to get more EM training data or validate transformation rules to get golden values. Since some of the human feedback obtained in one of the processes can effect the other, treating these processes holistically, not consecutively, by smartly scheduling questions, has the potential to significantly improve the quality of golden-records.  For example, given two records, \texttt{Massachusetts Institute of Technology, 77 Mass. Avenue, Cambridge, MA} and \textit{MIT, 77th Massachusetts Ave, Cambridge, Massachusetts}, existing EM tools will take them as non-matching pair, because they have small textual similarity. However, if we use transformation rules to transform 77th to 77,  Mass. to Massachusetts, and Ave to  Avenue, then we can easily match the two records. Moreover, we can infer a new transformation rule:   Massachusetts Institute of Technology $\rightarrow$ MIT.



%Traditional machine algorithms contain the following steps. 

\subsubsection{Entity Matching Question}

For each entity matching question $\qm$ that is not pruned by blocking rules, we use the entity matching tool (e.g., random forest) to compute a probability that the pair is a matching pair $Pr(\qm)$. The larger $Pr(\qm)$ is, $\qm$ has a larger possibility to be matching. The smaller $Pr(\qm)$ is, $\qm$ has a larger possibility to be non-matching.  However, if $Pr(\qm)$ is close to 0.5, the entity matching tool cannot discriminate it clearly, and we want to ask the human to label such pair and use its answer to enhance the entity matching tool. To this end, we define the uncertainty of a pair $U(\qm)$ as follows.
\begin{equation}
U(\qm)=-\Bigl(\log Pr(\qm) + \log\bigl(1-Pr(\qm)\bigr)\Bigr)
\end{equation}

We sort the pairs by the uncertainty in ascending order and select the pairs in this order. 

\lgl{too expensive}

%\lgl{add an example}\qr



%we want to know whether they have correlations. W
%e.g., \qt and \qm, and compare four cases. (1) We run the machine algorithms based on the answers of one questions (\qt or \qm). (2) We run the machine algorithms based on the answers of one questions (\qt or \qm). 
%\subsection{Question Selection from Different Question Types}

%Note that it is hard to compare questions from different types, especially comparing repairing questions and entity matching questions. To this end, we introduce an estimation-based method that estimates the benefit of each question and selects the question with the largest benefit. 

%\#affected matching pairs? 

%\hi{Selecting The Best Question in Each Round.} Formally, we first get a sample of records and label the records by expert to get the ground truth of their golden records. Next we run an iterative method to select questions. Initially, we select the best question from each set. Then for each question, we ask the human to label the answers and run the machine algorithms to get the golden records. Next we compute the quality improvement on these sample records. We call the quality improvement as the benefit, denoted by $\mathcal{B}$. We identify the question with the largest benefit and select the next question from the same set.  Iteratively, we can select questions within the budget. Note that after running the machine algorithm in each round, we will re-select the four question sets based on the new results. 

%\hi{Selecting $b$ Questions in Each Round.} We can also select multiple questions in each round to reduce the machine time. In each round, we compute the benefit of each question, and then we proportionally select the questions. Formally, suppose we select $b$ questions in each round, and suppose the average benefit improvements of the four questions types are respectively $\mathcal{B}_T,\mathcal{B}_M,\mathcal{B}_C,\mathcal{B}_R$, next we select $b\cdot\frac{\mathcal{B}_T}{\mathcal{B}_T+\mathcal{B}_M+\mathcal{B}_C+\mathcal{B}_R}$ training questions, $b\cdot \frac{\mathcal{B}_M}{\mathcal{B}_T+\mathcal{B}_M+\mathcal{B}_C+\mathcal{B}_R}$ entity matching questions,  $b\cdot\frac{\mathcal{B}_C}{\mathcal{B}_T+\mathcal{B}_M+\mathcal{B}_C+\mathcal{B}_R}$ clustering questions, and $b\cdot\frac{\mathcal{B}_R}{\mathcal{B}_T+\mathcal{B}_M+\mathcal{B}_C+\mathcal{B}_R}$ repairing questions. In this way, we only call the machine algorithms $\frac{B}{b}$ times. Note that the questions in the same question set may influence each other. For example, after asking the best EM question, the question order in the EM question set may be changed as the EM tool is updated. To address this issue, we need to consider the ``influence'' when selecting multiple questions from a set. For example, consider selecting $x$ EM questions. We first select the best one. Next we check whether the second one has the same feature with the first one, i.e, both the two questions have high similarity on the same attribute. If yes, we skip the second and check the third; otherwise we select it. In addition, the questions from different question sets may have ``overlap''. For example, if a clustering question and a training rule question cover the  same record pairs,  we do not want to keep both of them. To address this issue, we first select the questions from the set with the largest benefit. Next we select the questions from the set with the second largest benefit as follows: when selecting a question, if the question has large overlap with those selected questions, we skip the question; otherwise we select it.



%question assignment based on the benefit

%In each round, it selects $b$ questions \Qb, asks human to answer the $b$ questions, uses the human feedbacks to generate some training data (for questions in $\mathbb{Q}_T$ and $\mathbb{Q}_C$) and repair the dataset $D$ (for questions in $\mathbb{Q}_R$), runs the machine algorithms, and generates new $\qt, \qc, \qr$. Next it estimates the benefits of each question in $\Qb$ questions using all the questions that have been answered in previous rounds,  and uses the benefits to select $b$ questions from new \Qall in next round. 

%We first discuss how to select the best question from the four question sets and then present how to select the best one from  the four selected questions.



%\section{Benefit-based Question Selection} \label{sec:benifit}


%exploration-exploitation framework, which is an iterative method. In each round, the exploration step (called question selection) aims to select $b$ questions based on the asked questions while the exploitation step (called quality estimation) asks human to get the answers of the $b$ selected questions and estimates the quality improvement of these $b$ questions. 


%We use $Q_{C}$ to denote a cluster question and $\mathbb{Q}_C$ denote the set of clustering questions. 
% to get some matching pairs and feed them to the EM tool.
%, and the blocking rules, e.g., if the edit distance between two authors is larger than 10, then the two records do not refer to the same entity. We can use the matching rules to get some matching pairs and feed them to the EM tool. We can use the blocking rules to prune pairs that will not refer to the same entity. We use $Q_{T}$ to denote a training-rule question, \eg is $\phi_1$ a correct rule? and $\mathbb{Q}_T$ denote the set of training-rule questions. % questions that are approved by human.  We use $Q_{R}$ to denote a data repairing question and $\mathbb{Q}_R$ denote the set of data repairing questions. 
% on  and in this way, it generates a golden record for each cluster. 
%Data integration includes four key components: data preparation (\ie normalizing and cleaning data), schema integration (\ie lining up like attributes), entity matching (\ie finding clusters of records that represent the same entity), and entity consolidation (\ie merging each cluster into a ``golden record'', which contains the canonical or preferred values for each attribute).  In practice, these four processes are typically performed independently and consecutively: data preparation (DP), schema integration (SI), entity matching (EM), and finally entity consolidation (EC).
%We find that these components can be interleaved to benefit each other.  For example, entity matching can help data repairing, and entity consolidation can help entity matching. Next we present our observations that motivate our studied problem and proposed solution.

%During EM, human feedback is used to improve the quality of the clusters through:
%  focuses on improving the clustering quality by utilizing human feedback to 
%(1)~validating training rules to get more training data, 
%(2)~labeling more matching/non-matching pairs, or 
%(3)~validating clusters, \ie whether the records in the cluster refer to the same entity. 
%Each feedback has a different effect on improving the quality.  EC focuses on improving the quality of the golden records %in clusters by asking human to validate data transformation rules\mourad{It's better to refer to these as data transformation rules.}, 
%\eg transforming  \texttt{st} to \texttt{street} in an address attribute.
%\ie whether to apply data transformation  rules to a group of  records (\eg whether repairing \texttt{st} to \texttt{street} in address). 
%Theses components require to involve human. 
%Data repairing asks human to repair the data, 
%Note that some operations can be avoided, if they cannot change the result of computed golden records. 
%For instance, if repairing some errors cannot change the result of computed golden record based on the majority voting consensus, then this repair may not be needed. 
%Thus we need to 

%the user feedbacks about the canonical or preferred values within one cluster can be generalized (cf.~\cite{DBLP:conf/sigmod/HeVSLMPT16}) to other clusters. EM can get better clusters based on the normalized/repaired data.  Henceforth, these components should be interleaved, instead of being executed consecutively.

%\mourad{We first need to set the scene on the kind of EM/EC algorithms we're assuming.The concept of ``training rule'' for EM should be clarified.}


%\be
%	\itemsep-1mm\parsep-1mm
%	\item[(i)] {\em Data repairing helps entity matching.}
%	Entity matching are sensitive to data errors -- some duplicates cannot be detected, and some detected duplicates are false positives. Intuitively, the above cases can be alleviated if the data errors have been repaired.
%	\item[(ii)] {\em Entity matching helps data repairing.}   
%	We can first utilize entity matching to get clusters of records which have large possibility to be the same entity, and then repair the clusters. 
%	Postponing repairing to clusters might be cheaper than cleaning the entire data, because the records in the same cluster are very similar and we have more evidences  to identify the golden record.
%	% (\eg cluster-specific vs. columns-specific transformations in the {\em golden record} work).
%	\item[(iii)] {\em Entity consolidation helps data repairing.}
%	The user feedbacks about the canonical or preferred values within one cluster can be generalized (cf.~\cite{DBLP:conf/sigmod/HeVSLMPT16}) to other clusters.  Thus entity consolidation can improves the generality of data repairing. 
%	%\item[(iv)] {\em  Different operations are suitable for different types of errors.}  .
%	\item[(iv)] {\em Entity consolidation helps entity matching.} Since entity consolidation helps data repairing which in turns helps entity matching, entity consolidation can help entity matching. 
%
%\ee

%There are four possible ways to involve human to improve the machine algorithms. 
%
%(1) {\it Training Rule Question.} We can utilize high-quality training rules to improve the EM tool.  We consider both the matching rule, \eg rule $\phi_1$ if the Jaccard similarity of two paper titles is larger than 0.9, then the two records refer to the same entity, and the blocking rules, e.g., if the edit distance between two authors is larger than 10, then the two records do not refer to the same entity. We can use the matching rules to get some matching pairs and feed them to the EM tool. We can use the blocking rules to prune pairs that will not refer to the same entity. We use $Q_{T}$ to denote a training-rule question, \eg is $\phi_1$ a correct rule? and $\mathbb{Q}_T$ denote the set of training-rule questions. 
%
%(2) {\it Entity Matching Question.}  We can ask human to verify some entity pairs and feed the answers to the EM tool. For example, given two records ``Mike Stonebraker'' and ``Michale Stonebraker", we ask human to check whether they refer to the same entity.   We use $Q_{M}$ to denote an entity-matching  question and $\mathbb{Q}_M$ denote the set of entity-matching questions. 
%
%(3) {\it Clustering Question.} We can ask human to verify a cluster of records. If the records in the cluster do not refer to the same entity, the cluster is required to split into sub-clusters where all records in each sub-cluster refer to the same entity. Based on the answers of cluster questions, we can get some validated  matching pairs that are in the same cluster and some validated non-matching pairs that are from different sub-clusters. Then we can feed theses pairs to the EM tool. We use $Q_{C}$ to denote a cluster question and $\mathbb{Q}_C$ denote the set of clustering questions. 
%
%(4) {\it Data Repairing Question.}  We can ask human to validate a repairing question, where each question $v\rightarrow v'$ asks human to check whether the value $v$ should be repaired to another value $v'$ for all records containing value $v$. We repair the data using the repairing questions that are approved by human.  We use $Q_{R}$ to denote a data repairing question and $\mathbb{Q}_R$ denote the set of data repairing questions. 



%\stitle{Iterative Method.} Since interleaving the operations can improve the quality, 
%(e.g., data repairing can improve entity matching while high clustering precision can improve golden record), 
%we want to iteratively ask training rule, entity matching, clustering, repairing questions. Initially, we get four sets of questions, $\mathbb{Q}_T$, $\mathbb{Q}_M$,  $\mathbb{Q}_C$, and  $\mathbb{Q}_R$.  Next we select some questions from the four question sets, ask  human to get the results, and generate some training data (for questions in $\mathbb{Q}_T$, $\mathbb{Q}_M$,  $\mathbb{Q}_C$) and repair the dataset $D$ (for questions in $\mathbb{Q}_R$).  Next we call the machine algorithm using the new training data and the updated  datasets. We repeat the above steps until the budget is used up. Finally we can get the set $G$ of golden records.





%Traditional methods run entity matching, data repairing, and entity consolidation independently. Entity matching aims to find clusters of records that refer to the same entity. Data repairing detects and repairs the data errors. Entity consolidation merges each cluster and generates the golden record, which contains the canonical or preferred values for each attribute. However, these three components can be interleaved to benefit each other. We have the following observations that motivate our studied problem and proposed solution.

%We can select a set $Q_{R}$ of repairing questions
%Then we use the answers to feed the EM tool so as to improve the EM tool. 
%utilize active learning to select a set $Q_M$ of matching/non-matching pairs, e.g., whether iPhone X and iPhone 10 
%(4) Finally we run an EC tool (\eg majority voting) on each cluster to get a golden record for each cluster.   We first run a pre-trained EM tool (\eg random forests) to get a set of clusters  The matching/non-matching pairs can be gotten asked by asking human  (2)  


%A straightforward way selects questions in a round-robin strategy, i.e., select one question for each type in each iteration.  However this method cannot work well, because d 
%In each round, we judiciously select some questions to ask, get the answers, generate more training data or repair the data, and call the machine algorithm. 
% in multiple rounds. 
%Initially we run the traditional methods and get some questions. Then we select some question to ask the human and call the traditional method again using the answers of these questions.  Given a budget $\tau$, our goal is to effectively select the questions within the budget to maximize the quality (e.g., golden-record precision).
%We first use a matching training rule and an un-matching training rule to get some training data. Next we run the traditional solutions to generate the golden records. Then we can 

%In each round, we first run the EM algorithm by taking as input the answers of EM and CD questions in the previous rounds, and the repaired data by GR questions in the last round. Then we ask $x$ EM questions, $y$ CD questions, and $z$ GR questions, and run the single-round algorithm.  



%Hence, a natural question arises: {\em Can we interleave the above processes such that we can achieve a better data integration result but possibly with a lower cost?} : data preparation (\ie normalizing and cleaning data), schema integration (\ie lining up like attributes), entity matching (\ie finding clusters of records that represent the same entity), and entity consolidation (\ie merging each cluster into a ``golden record'', which contains the canonical or preferred values for each attribute).  In practice, these four processes are typically performed consecutively: data preparation (DP), schema integration (SI), entity matching (EM), and finally entity consolidation (EC). Moreover, at least 80\% human cost was spent on DP, EM, and EC. Hence, a natural question arises: {\em Can we interleave the above processes such that we can achieve a better data integration result but possibly with a lower cost?}



%Some operations (\ie the user picked canonical or preferred values in entity consolidation, transitivity in entity matching, and sample data errors and data repairs)  can be inferred and generalized.

%\stitle{Remarks.}
%Let's start by not making too many assumptions about what have been provided, and what the data will look like. Especially: (1) We don't assume that integrity constraints, data cleaning rules, positive/negative matching tuple pairs are provided, since these take $\sim$$80\%$ of the data integration cost.
%(2) We don't assume that there are only string standardization problems within clusters of duplicates.  Instead, we consider both canonical values (\eg from {\em Prof.} to {\em Professor}) and preferred values (\eg the {\em Professor} title should be preferred than an {\em Associate Professor}). 





%This traditional method has some limitations. First, the majority voting based method may not work well, because there may not exist a correct value, and it requires to merge the attribute values from multiple records and even pair the data to improve the quality. Second, the clusters may be not accurate, e.g., records in a cluster do not refer to the same entity or a cluster misses some records that should be in this cluster, and thus it requires to improve the cluster quality. Third, the data repairing can also improve the entity matching.  Fourth, improving entity matching can also enhance entity consolidation.







\iffalse

\stitle{Naive Method 1.} In each round, we ask $\tau$ EM, $\tau$ CD, $\tau$ GR questions, where $\tau \in [1,5]$.


\stitle{Naive Method 2.} 
In the first round, we ask 1 EM, 1 CD, 1 GR question, and evaluate the benefit of each question (the evaluation is hard which will be discussed later). In the next round, we double the number of ``most beneficial'' questions and halve the number of other questions (keeping at least one question for each question type).  For example, if CD is the most beneficial question in the first round, we ask 1 EM, 2 CD, 1 GR in the second round. Then if GR is the most beneficial question in the second round, we ask 1 EM, 1 CD, 2 GR in the third round. 
 

\stitle{An Optimization Method.} In each round, we first select a single question $q\in Q_{EM}\cup Q_{CD} \cup Q_{GR}$, and then pack the questions into a question set $Q$. Next we run the single-round algorithm based on $Q$. 


\stitle{Step 1: Select a single question $q$.} 
An ideal method enumerates every possible question $q$, asks the human to get the answers $A_q$, reruns our method to get the new golden records $\gq$, evaluates the quality improvement $f(\gq|G)$ of golden records $\gq$ given the current golden record $G$, and selects the question to maximize $f(\gq|G)$. 

There are two challenges. First,  we cannot ask the human for every question since it is cost expensive, and we only want to ask the questions with high benefit-cost ratios.  Second, we have no ground truth data and it is rather hard to quantify $f(\gq|G)$. Next we give the basic idea to select beneficial questions. 

To address these challenges, we can evaluate the benefit of the three types of questions respectively. 

For EM, $q$ is a beneficial EM question if it can improve the GR precision. However it is hard to evaluate the improvement. Instead, we evaluate whether it can improve the clustering precision, because enhancing clustering precision can indirectly improve the GR precision.
If we have the answer of $q$, we can estimate the clustering improvement by computing the number of affected clusters through running the EM tool with the answer of $q$. However it is hard to get the answer of $q$ if we do not ask the human. We have several strategies to address this issue. (1) We use the number of affected clusters in the last round to quantify the benefit. (2) We predict the answer of $q$ and run the EM algorithm based on the predicted answer to get the number of affected clusters. (3) We can also utilize the traditional active learning techniques to select EM questions (the pairs between the matching and non-matching pairs).

Similarly, for CD, $q$ is a beneficial CD question if it can improve the clustering precision. Since we do not know how a cluster w.r.t. $q$ will be split, we still need to use the above  methods to quantify the benefit. 


For GR,  $q$ is a beneficial GR question if it can improve the GR precision. If the GR question has a large frequency and can be applied to many records, then it has large possibility to improve the GR precision. We can use the frequency to quantify the benefit. However we do not know whether the rule will be approved by the human, and we either predict its answer or use the results in the last round. 

We will design more effective models to quantify the benefit of a question.


\stitle{Step 2: Pack questions to a set $Q$.}  Initially we call Step 1 to get the first question $q$ and set $Q=\{q\}$. We then  iteratively call Step 1 to get next question $q'$. If $q'$ can be packed into $Q$, we add $q'$ to $Q$; otherwise we terminate. 



\stitle{Step 3: Run the single-round method with $Q$.} We run the single-round algorithm with the questions in $Q$. 

 
\stitle{Stop Condition.}  If a budget $B$ is given, once the budget runs out, the algorithm terminates. If there is no budget, when the quality improvement is small (e.g., $f(\gq|G)<\epsilon$), the algorithm terminates. 


\ctitle{Observations to question selection.} \lgl{(1) If the clusters have low precision, we want to select CD questions to split the clusters; otherwise CD questions will not improve the quality. (2) If the clusters have low recall, we want to select EM questions to merge the clusters. (3) If majority voting cannot select good attribute values (e.g., the attribute values in many clusters have large uncertainty),  we want to select GR questions. If the frequency of a GR rule is low, asking the GR question has limited benefit.  We need to propose a model to quantify the improvement of a question.}


\ctitle{Discussion.} \lgl{Do we need to pack the questions? The upside of packing is to reduce the number of rounds so as to reduce the latency. Is the latency important in our problem? The downside of packing is to potentially ask some non-optimal questions. For example, given two questions $q$ and $q'$. If we first ask $q$ and run the single-round algorithm, then we may select other questions instead of $q'$. So if we want to pack multiple questions together, we need to guarantee that (1) after running the single-round algorithm with $q$, we will still select $q'$ in the next round; (2) running the single-round algorithm twice with $q$ and $q'$ as input respectively will get the same result as running the single-round algorithm once with both $q$ and $q'$ as input. }

\fi







































%(i) Entity matching are sensitive to data errors -- some duplicates cannot be detected, and some detected duplicates are false positives.  Intuitively, the above cases can be alleviated if the data errors have been repaired.
%(ii) Postponing data cleaning to clusters might be cheaper than cleaning the entire data (\eg cluster-specific transformations vs. columns-specific transformations in the {\em golden record} work).

%Clusters generated from entity matching can provide more evidences for the tuples in the same cluster, and data cleaning on a cluster of highly similar tuples can improve the quality of error detection and data repairing.  Furthermore, some data cleaning algorithms on clusters (\eg data transformations) is cheaper than on the entire data.
%For example, if some redundant and similar examples are feed into the entity matching, the quality cannot be improved. 
%\be
%	\item Entity matching are sensitive to data errors -- some duplicates cannot be detected, and some tuples that are computed as duplicates are not duplicates. 
%	
%	and some tuples are mistaken as the same entity, leading to some low-quality clusters. Data cleaning can improve the data quality, and thus can help find better clusters.
%
%	\item Clusters generated from entity matching can provide more evidences for the tuples in the same cluster and data cleaning on a cluster of highly similar tuples can achieve  higher quality.  Furthermore, data cleaning on clusters (\eg data transformations) is cheaper than on the entire data. 
%
%	\item Some data cleaning and entity matching operations can be avoided, if they cannot change the result of computed golden records (for goal-oriented data cleaning). For example, if some redundant and similar examples are feed into the entity matching, the quality cannot be improved. 
%
%	\item Some operations (\ie the user picked canonical or preferred values in entity consolidation, transitivity in entity matching, \lgl{how about data cleaning})  can be inferred, so as to produce more generalized rules or integrity constraints.
%\ee

%Data cleaning can help find better clusters, and better golden records. (2) Sometimes, d%
%(5) We rerun the EM tool on the repaired data to generate the clusters. \lgl{We can either put Step 5 here or take it as the Step 1 in the next round. The difference is whether we run EM again after asking GR questions and before EC.} 


%\stitle{Discussion 1.} \lgl{We may want to discuss which architecture we want to use.}


%%%%%%%%%%removed%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%Assume that at round $i$, we have budget $B_i$.
%We use $B_i/2$ for testing which step, EM, CD or GR, is the most significant for this round. 
%We then use the following $B_i/2$ budget all for this step.
%
%That is, we use $B_i/6$ for EM, $B_i/6$ for CD and $B_i/6$ for GR, and evaluate the significance of these answers.
%If $CD$ is the most impactful, we then ask $B_i/2$ CD questions.
 


\iffalse

  be the set of all generated questions. {\bf Question Scheduler} selects questions $q\in Q$

There are several challenges in this problem. 

(1)  How to decide the number of EM, CD, GR questions?

(2) 



%In each round, we select $x$ EM questions, $y$ CD questions, and $y$ GR questions.

\stitle{Step 1: Cold Start.}  
Given a dataset $D$, we first run a pre-trained EM tool (\eg random forests) to get a set of clusters, and then run an EC tool (\eg majority voting) to get a set of golden records. 

%Note that EM and EC also output a set of questions $Q_M$ and $Q_C$ to the human.  For EM, we can use active learning to generate $Q_M$, where each question in $\QM$ is a record pair that asks human to check whether they are duplicates or not. For EC, each question is a cluster of records, which asks human to select a golden record, or a golden value for a specific column.


\stitle{Step 2:  Question Generation.}  For EM,  we use an active learning model of an EM tool to select a set $Q_{EM}$ of EM questions, which can be used to improve the EM accuracy. For CD, we can select a set $Q_{CD}$ of cluster debugging questions, which can be used to improve the clustering accuracy. For GR, we can select a set $Q_{GR}$ of golden record questions, which can be used to improve the GR  accuracy. 


%After getting the answers of the questions in $\QM$ and $\QC$ from human, there are several cases that the basic pipeline in Step 1 will be affected.  (i) Given the clusters ${\bf C'}$ from EC (${\bf C'}$ could be the same as or a modification of ${\bf C}$), a DR tool can be invoked (\eg cluster-specific data transformation) to repair the data, which will trigger $EM$ and $EC$ to be reevaluated.  (ii) A DR tool can be invoked to apply directly on the input data $D$, which will affect the downstream $EM$ and $EC$. (iii) An active learning model of an EM tool can select more questions, after being verified by the user, to improve the accuracy of the EM tool, which will affect the generated clusters ${\bf C}$. Naturally, EC will be reevaluated.

%In any case (i, ii and iii) above, there are different questions raised by different components. Which question to answer first will be discussed below.

%Given the clusters $C'$ generated from the EC tool, a DR tool utilizes the clusters to repair $D$ and outputs a repaired data $D'$. The DR tool also generates a set $Q_R$ of repair questions that ask the human to check whether applying these repairs.  In this work, we take the transformation rule as an example, where each repair question asks whether we change $c$ to $c'$ in this cluster. 

\stitle{Step 3: Question Scheduler.}   
Let $Q=Q_{EM}\cup Q_{CD} \cup Q_{GR}$ be the set of all generated questions. {\bf Question Scheduler} selects questions $q\in Q$. Let's start simple by considering one question only (\ie $|q| = 1$), and we will discuss more general case later (\ie $|q|>1$).  Based on the selected question(s), we get the answer $\aq$, and rerun the tools to get new golden record $G=\gq$.  Our algorithm repeats to call  {\bf Question Scheduler} until the stopping criterion is satisfied. 

\fi

%for each question $q\in Q$, we predict its answer $\aqhat$, run the three tools to get a set of golden records $\gqhat$, evaluate the quality improvement $f(\gqhat|G)$ of golden records $\gqhat$ given $G$, and select the question $q$ with the maximal quality improvement, i.e., maximizing $f(\gqhat|G)$.

%We select the question $q$ with the maximal quality improvement, i.e., maximizing $f(\gqhat|G)$. 




%(We will discuss how to select $k$ questions to ask in parallel, e.g., $q$ is a set of $k$ questions.) Based on the question $q$ and the answer for $q$ gotten from the human, we rerun the tools $DR, EM, EC$ in order.  

\iffalse
\vspace{-.25em}
\subsection{Challenges}
\vspace{-.25em}

\ctitle{Challenge 1.} How to predict the answer of $q$? 

\ctitle{Hint 1.} We can propose a probability model. For EM, we can utilize the similarity to estimate the probability whether a candidate pair is a matching pair. For DR, we can use the frequency to estimate the probability whether a candidate repair is correct. For EC, we can use majority voting to select the golden record.  

\ctitle{Challenge 2.} How to compute golden record $\gqhat$ based on the predicted answer of $q$? 

\ctitle {Hint 2.} We design incremental algorithms that only compute a subset of data (or {\em affected area}). 

\ctitle{Challenge 3}  How to evaluate the golden record set $\gqhat$, i.e. computing $f(\gqhat|G)$?

\ctitle{Hint 3.} We can compute the clustering quality based on some criterions. 

\ctitle{Challenge 4.} How to select $q$ from $Q$ if $Q$ is large? How to avoid rerunning the three tools  for each $q\in Q$ to compute $\gqhat$ on the entire data? 

\ctitle {Hint 4.}  We can share the computations on different $q$'s. We can also use an estimation-based method to estimate $\gqhat$ without rerunning the tools. For each tool, we can define a benefit model to ask $q$. For DR, we estimate how many tuples will be repaired by $q$. For EM, we estimate how many pairs will be changed from mismatching to matching  by $q$ (and vice versa). For EC,  we estimate how much the uncertainty will be reduced by $q$ in every cluster.

{\bf We can also refine our prediction model based on the answer $\aq$ of selected/asked questions $q$, by comparing $\aqhat/\aq, \gqhat/\gq, f(\gqhat|G)/f(\gq|G)$.}


\section{Preliminary}

\section{System Overview}

\section{Predicting Answer of Question {\large $\lowercase{q}$}}

\section{Computing Golden Record {\large $\hat{G}$}{\large $\lowercase{q}$}}

\section{Evaluating Quality Improvement {\large $\lowercase{f}$}({\large $\hat{G}$}{\large $\lowercase{q}$}|{\large $G$})}

\section{Efficiently and Efficiently Selecting Question {\large $\lowercase{q}$}}

\section{Extension to {\large $|\lowercase{q}|>1$}}

\section{Experiments}





\fi

%\newpage


\iffalse
\begin{figure}[!t]%\vspace{-1em}
\begin{center}
\centering
\includegraphics[width=0.3\textwidth]{figs/ex-order2.eps}
\vspace{-1em}
\caption{A running example \label{fig:ex:1}}
\end{center}
\vspace{-1.75em}
\end{figure}
\fi








%Computing Golden Record {\large $\hat{G}$}{\large $\lowercase{q}$} for {\large $\lowercase{q}$} in {\large $Q$}

%(1) {\em Optimize the 80\%, not 20\%.} 
%Do not make assumptions about what have been provided such as integrity constraints, data cleaning rules, positive/negative matching tuple pairs -- these take 80\% of the data integration cost.
%(2) {\em Start by a general problem.} Do not assume what the data will look like; for example, in a cluster of duplicates, we consider both canonical values (\eg from {\em Prof.} to {\em Professor}) and preferred values (\eg the {\em Professor} title should be preferred than an {\em Associate Professor}). \lgl{I cannot follow the remarks!}


%\begin{definition}[Data Repairing] Given a table $D$ integrated from multiple data sources, data repairing aims to repair an incorrect value $v$ to a correct value $v'$. 
%\end{definition}

%solve the problem of data integration, namely given a the table $D$,
%\lgl{add an example: shown as table \ref{gr_example}, we take the entry offered by Google map as the correct record.}




\subsection{Machine Modules}

We utilize the following machine modules to compute golden records.


\hi{(1) Entity Matching.} Based on table $D$, it aims to generate a set $P$ of matching pairs. Any entity-matching tool can be used to generate $P$, and here we take the machine-learning based method (\eg random forest) as an example. It first gets a set $T$ of training data and trains an EM model. Next it uses blocking rules to remove the pairs that have low possibility to be matching and get a set of candidate matching pairs. Then it utilizes the trained EM model to identify the matching pairs from the candidate set. In Table~\ref{example},  if we use a training rule, if $Jaccard(Name)\ge 0.6$ then matching, then there are  4 clusters, $(r_1,r_2), (r_3,r_4), (r_5,r_6), (r_7,r_8)$.  If the rule is $Jaccard(Address)\ge 0.5$ then matching, all records are clustered into the same cluster. If the rule is the same Zipcode then matching, there are 2 clusters in Figure~\ref{gr_example}.


 %It can also use active learning to select some ``hard'' pairs that are hard to discriminate by the model (\eg the EM model return that the pairs have 50\% probability of matching pairs and 50\% probability of non-matching pairs), asks the human to check the pairs in order to get more training data and uses the training data to improve the training model.


\hi{(2) Entity Clustering.} Based on the set $P$ of matching pairs, it groups the entities into clusters such that two records $r_1,r_2$ in the same cluster if and only if $(r_1,r_2)\in P$.  This step gets a set $C$ of clusters. In Figure~\ref{fig:ex:1}, for the left figure there are two clusters based on the matching pairs: $\{r_1,r_2,r_3,r_7,r_8\}$ and $\{r_4,r_5,r_6\}$.



 \hi{(3) Entity Consolidation.}  For each cluster $c\in C$, it aims to generate a golden record $g$ and add it into the set $G$. Assume there are $x$ records $r_1,r_2,\cdots, r_x$ in the cluster. It generates the golden record by selecting the majority value of each attribute. For example, for the $i$-th attribute, it selects the majority value in this attribute as the golden attribute value. Then the golden record is composed of the golden values on each attribute in the cluster.  In Figure~\ref{fig:ex:1}, considering cluster ${r_1,r_2,r_3}$ in the middle figure, the voted value on the Name attribute is MIT Electrical Engineering and Computer Science.



The machine-only algorithms usually cannot produce high-quality golden records because the data is rather dirty and it requires to involve human to improve the quality.  For example in the cluster of $\{r_1, r_2, r_3, r_7,r_8\}$, the data is rather dirty and the voting based method cannot obtain the golden value without data normalization/repair.


%For example, Figure~\ref{fig:ex:1} shows an example. It first 
%Table~\ref{table:ex:naive} shows the results of the machine algorithms. We can see that the clusters generated are not correct and the golden values are not correct. 

\subsection{Human Operations}


\begin{table}[!t]
\centering
\caption{Notations \label{table:notation}}
\begin{tabular}{|l|l|}\hline
Notation & Description \\ \hline
$P$ & A set of matching pairs\\\hline
$C$ & A set of clusters\\\hline
$\qt(\Qt)$ & A (set of) training rule question \\\hline
%$\qm(\Qm)$ & An (set of) entity matching question\\\hline
$\qc(\Qc)$ & A (set of) clustering question \\\hline
$\qr(\Qr)$ & A (set of) transformation question\\\hline
$\mathcal{C}_T$ & The cos of training rule question $\qt$ \\\hline
%$\mathcal{C}_M$ & The cos of entity matching question $\qm$ \\\hline
$\mathcal{C}_C$ & The cos of clustering question $\qc$ \\\hline
$\mathcal{C}_R$ & The cos of transformation question $\qr$ \\\hline
\end{tabular}
\end{table}


We utilize the following human operations to improve entity matching and entity consolidation.

\subsubsection{Training Rule Validation} 

To improve entity matching, we can use training rules to get more training data and feed them to the entity-matching tool to improve the EM  quality. However it is hard to get 100\% accurate rules and we ask human to validate the rules. If the rules are approved, we take the record pairs that satisfy the rule as training data and re-train the EM model.

\hi{Training Rule Validation Question.} Formally, a matching (non-matching) rule question $\qt$ includes an ``if-condition-then-matching (non-matching)'' clause as well as several records pairs that satisfy the rule.  For example, $Jaccard(Name)\ge 0.5$ is a matching rule and $Jaccard(Address)\le 0.1$ is a non-matching rule. To help human validate a training rule, we also associate a sample of entity pairs  that satisfy the rules (\eg 10 pairs).  We use \qt to denote a training rule and \Qt to denote the set of training rules.


% and $|\Qt|$ to denote the size of $\Qt$, i.e., the number of pairs satisfying the rule.
%We ask the human to verify the rule, and human requires to check the entity pairs 
%and label the matching-pairs and non-matching pairs. Then these results are taken as the training data. 
%\lgl{For example, consider the matching rules $Jaccard(street)\ge 0.6$. *** satisfy the rules and are taken as the positive examples.}


\hi{Training Rule Generation.} The training rules can be hand-crafted by domain experts or the rules learned from random forest (i.e., the leaf nodes in the random forest). 

For example, Table~\ref{fig:tr:ex} shows 3 training rule examples. The rule: if the same Zipcode then matching, will take all the records with the same Zipcode as matching pairs.


\begin{figure}[!t]
\begin{center}
\centering
\begin{tabular}{|p {12em} | p {8em} |l|}\hline
Rule & 3 examples & Results \\ \hline
If $Jaccard(\texttt{Name})\ge 0.5$ then Matching & $(r_1,r_2), (r_3, r_4)$, $(r_5, r_6)$& Yes\\\hline
If $Jaccard(\texttt{Address})\ge 0.5$ then Matching & $(r_1,r_2), (r_3, r_4)$, $(r_7, r_8)$& Yes\\\hline
If same $\texttt{Zipcode}$ then Matching & $(r_1,r_2), (r_1, r_7),$ $(r_7, r_8)$& Yes\\\hline

\end{tabular}
\vspace{-.5em}
\caption{Training Rules\label{fig:tr:ex}}
\end{center}
\vspace{-1.5em}
\end{figure}







%%%%%%%%%%%Remove EM questions%%%%%%%%%
\iffalse

\subsubsection{Matching Pair Validation} 

To improve entity matching, we can use active learning to select entity pairs, ask the human to validate the pairs, and feed them to the entity matching tool to improve the matching quality. 

%We require to ask the human to validate the pairs. 


\hi{Entity Matching Validation Question.}  Formally, an entity matching question $\qt$ is a pair of records. We ask human to verify whether the pair refers to the same entity. Then the result is taken as the training data. Obviously $|\Qm|=1$.


\hi{Entity Matching Question Generation.} All the pairs can be taken as an entity matching question. However there are huge number of pairs. To address this problem, we can use active learning to select record pairs. The basic idea is that for each record pair, it utilizes the entity matching tool to compute a probability whether the pair is a matching pair. If the probability is close to 0.5, the entity matching tool cannot  discriminate it and will take it as an entity matching question. We will introduce the details in Section~\ref{sec:benifit}.

%Based on the matching pairs returned by the entity matching tool, we can compute a similarity threshold that is around the matching pairs and non-matching pairs. For each pair, we compute a similarity, which is the average similarity on each attribute. We can use any similarity functions, e.g., Edit distance, Jaccard. Then we take the smallest threshold among all the pairs as the similarity bound. Then we can select the top pairs smaller than the bound as matching questions. 

For example, the EM tool cannot discriminate $\langle r_5, r_6\rangle$ clearly and we want to ask this pair to train a more effective model. 

\fi 
%%%%%%%%%%%Remove EM questions%%%%%%%%%



\begin{figure}[!t]
\begin{center}
\centering
\begin{tabular}{|l | l |}\hline
Rule & Results \\ \hline
\{$r_1,r_2,r_3,r_7,r_8$\} & No: $\{r_1,r_2,r_3\}$; \{$r_7,r_8$\}\\\hline
\{$r_4,r_5,r_6$\} & No: $\{r_4\}$; \{$r_5,r_6$\}\\\hline
$\{r_5,r_6,r_7,r_8\}$ & Yes \\\hline

\end{tabular}
\vspace{-.5em}
\caption{Cluster Questions\label{fig:tr:ex}}
\end{center}
\vspace{-1.5em}
\end{figure}



\subsubsection{Clustering Validation} 

The EM model may generate incorrect clusters. To improve cluster quality,  we can ask human to verify a cluster of records. If the records in the cluster do not refer to the same entity, human is required to split the records in the cluster into several sub-clusters where all records in each sub-cluster refer to the same entity; otherwise, all the records in the cluster are verified to be matching.


\hi{Clustering Validation Question.}  Formally, a clustering question $\qc$ is a cluster of records. We ask   human to verify whether the pairs in the cluster refer to the same entity. If the records do not refer to the same entity, the human requires to spilt the cluster into $C_1, C_2,\cdots, C_y$ clusters.  Then the pairs in the same cluster can be taken as matching pairs and the pairs from different clusters can be taken as non-matching pairs, and these results are taken as the training data. 
We use \qc to denote a clustering question and \Qc to denote the set of clustering questions.
%Here $|\qc|$ is the number of records in the cluster.


\hi{Clustering Question Generation.}  All the clusters generated by the EM model can be taken as a cluster question. 

For example, Table~\ref{fig:tr:ex} shows 3 clustering questions.  Cluster \{$r_1,r_2,r_3,r_5,r_7,r_8$\} in Figure~\ref{fig:ex:1} can be chosen as a cluster question, and human can discriminate address of MIT EECS from MIT Computer Science, and split the cluster into two sub-clusters: one for EECS and the other for Computer Science. 

\begin{figure}[!t]
\begin{center}
\centering
%\includegraphics[width=0.5\textwidth]{figs/gr-example.eps}
\begin{tabular}{|l|l|l|}\hline
Rule & 3 Examples & Results  \\ \hline
\#th $\rightarrow$ \# (\# is a numerical value) & $r_3,r_5,r_7$ & Yes\\\hline
Street $\rightarrow$ St & $r_4,r_8$ & Yes\\\hline
\end{tabular}
\vspace{-.5em}
\caption{Transformation Rules\label{fig:gr-example}}
\end{center}
\vspace{-1.5em}
\end{figure}



\subsubsection{Transforamtion Rule Validation} 

In some cases, there may not exist majority values in an attribute, it requires to normalize/repair the data to improve the quality of golden records. Here we use the transformation rule as an example to repair the data. A rule $v\rightarrow v'$ repairs the records with value $v$ to the value $v'$. We can ask human to validate the rule. If the rule is approved, we use the rule to repair the data. 


\hi{Transformation Validation Question.}  Formally, a transformation validation question $\qr$ is a transformation rule $v\rightarrow v'$ as well as a sample of records with value $v$. We ask the human to verify whether repairing rule can be applied to the records. If the rule is approved, we pair the records and update the dataset $D$. 
%Here $|\Qr|$ is the number of records in the rule. %We ask the human to identify the records that can be applied for the rule. 
For example, Figure~\ref{fig:gr-example} shows several transformation rules. \#th(nd) $\rightarrow$ \# will transform a numerical value with th(nd) to the numerical value, e.g., 50th to 50 and 32nd to 32.

% consider three repairing rules: ${Capital[2]}digit[+] \to {Capital[2]}$ can be applied to $MASSACHUSETTS \to MA$ and $CALIFORNIA \to CA$. Rules $Avenue \to Ave$ and $boulevard \to blvd$ can be applied to the street column.

\hi{Transformation Question Generation.}  For each cluster, on each attribute, we align the attribute values as follows. We first get some matching tokens and then split the attribute value based on the matching tokens and generate some segments. Then for each segment pair $(v, v')$, we generate a repairing rule. We can also group the repairing rules for different pairs and each repairing rule includes all the corresponding records containing $v$. Thus $|\qr|$
is the size of records associated with the rule \qr. Please refer to \cite{DBLP:journals/corr/abs-1709-10436} for more details of transformation rule generation. 

%For example, Figure~\ref{fig:gr-example} shows several transformation rules.




\subsection{Human-in-the-loop Data Integration}


%Given a set of training rule questions \Qt,  a set of clustering questions \Qc, and a set of transformation questions \Qr,  and 

Given a budget to ask human, we aim to select a sequence of questions $\Qs=\langle Q_1,Q_2, \cdots, Q_B\rangle$ to ask human in order to maximize  the accuracy of golden records, where $Q_i$ is either a training rule question, clustering question or transformation question. 


%For each question, it asks human to get the answers, runs the machine algorithms, and asks the next questions. Iteratively, it can get the golden records. 


Initially, we need to run the machine algorithms to generate question sets \qt, \qc, and \qr. Toward this goal, we require to get some training data to train the EM model. We select several training rules to get such training data (we will discuss the details on how to select training rule questions in Section~\ref{subsec:sorting}). Then we run the machine algorithms to generate the clusters and infer the golden records. In this way, we can generate three sets of questions, $\mathbb{Q}_T$, $\mathbb{Q}_C$, and  $\mathbb{Q}_R$.  Let $\Qall = \Qt\cup \Qc\cup \Qr$ denote the set of all possible questions. 

Next a brute-force question scheduling method enumerates every $B$-size permutation of $\Qall$, computes the golden-record quality (after asking these questions, getting answers, and re-running the machine algorithms), and selects the permutation with the largest quality as \Qs. However this method has several challenges.

\hi{Challenge 1: Question Sequence Enumeration.} It is prohibitively expensive to enumerate all permutations of $B$-size subsets of $\Qall$.

\hi{Challenge 2: Golden-record Qualtiy Computation.} It is rather hard to compute the golden-record quality of a question sequence, because $(i)$ we do not know the ground truth of golden records, and $(ii)$ we do not know the human answer of each question before we ask the questions. 


\hi{Challenge 3: Questions have correlations.}  Selecting a question may affect the clusters and golden records, and thus affect other questions. So \Qall will dynamically changes after asking some questions. We cannot select a static set of questions \Qs in a single round. Instead, we aim to first select several questions,  use the human feedback of these questions to compute the clustering quality and golden-record quality, and then guide us to select the following questions. 


To address the above challenges, we propose an iterative estimation based method. The basic idea is that it selects $b$ questions in each round, uses the human feedback of these $b$ questions to estimate the benefit of each question (and a question sequence), and then utilizes the benefits to select $b$ questions in next round. We will present the details in the next section.


%It is rather hard to compute the golden-record quality of a question sequence, because $(i)$ we do not know the ground truth of golden records, and $(ii)$ we do not know the human answer of each question before we ask the questions. 











\iffalse
We first use several matching training rules and non-matching training rules to get some training data. Next we run the machine algorithms to generate the golden records. Then we can get four sets of questions, $\mathbb{Q}_T$, $\mathbb{Q}_M$,  $\mathbb{Q}_C$, and  $\mathbb{Q}_R$. 
Next we select some questions from the four question sets, ask the human to get the results, and generate some training data (for questions in $\mathbb{Q}_T$, $\mathbb{Q}_M$,  $\mathbb{Q}_C$) and repair the dataset $D$ (for questions in $\mathbb{Q}_R$).  Next we call the machine algorithms using the new training data and the updated  datasets. We repeat the above steps until the budget is used up. Finally we can get the set $G$ of golden records.

\lgl{add pseudo code here}

\lgl{refine the examples}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]\vspace{-1em}
\begin{center}
\centering
\includegraphics[width=0.5\textwidth]{figs/odi4.eps}
\vspace{-1.5em}
\caption{Question Selection Framework\label{fig:arch4}}
\end{center}
\vspace{-1.5em}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

One big challenge here is to select ``high-quality'' questions.  A straightforward way selects questions in a round-robin strategy, i.e., select one question for each question type in each iteration.  However this method cannot work well, because different questions have different cost and benefit. For example, training rule questions, entity matching questions and clustering question can improve the cluster quality, while the date-repairing question can improve the golden record accuracy. Thus, we need to judiciously select questions to maximize the golden-record quality.  Figure~\ref{fig:arch4} shows the framework of question scheduling and Figure~\ref{fig:rex} shows a running example. \ji{ [Ji modified] Initially, we know nothing about the cluster, tuples are separated completely, in this case, the best choice is using validated rule to improve the recall of the cluster. After applying rule Jaccard(street) $\ge$ 0.5, $r_{9}, r_{10}$ are incorrectly classified into the first cluster as their addresses are too close to tuples in the first cluster. There are three errors now, we can not reduce rule threshold to connect $r_{9}r_{11}$ or $r_{5}r_{6}$ because that would bring more harm than benifits, and we can not ask repairing question because nonsense questions like $77\to1400$ would be chose as repairing question at this moment. Therefore, we choose cluster question to split $r_{9}$ and $r_{10}$ from the first cluster. All the university names and their abbreviations appear in same clusters now, and we can repair all these in one slot by asking repairing question, the red circles indicate the tuples whose name is modified. Machine will connect $r_5$ and $r_6$ because of same name. At last, add validated rule Jaccard(name) $\ge$ 0.5 to connect $r_9$ and $r_{11}$ and add them into training data to train new model.} $r_{5}, r_8$ should be merged with $r_6$ and $r_7$. $r_9, r_{10}$ should be merged with $r_{11}$ and $r_{12}$. Then in the first round, we select a cluster question $Q_C$ for cluster \{$r_1,r_2,r_3,r_4, r_{17}, r_{18}$\}, and it is split into two clusters  \{$r_1,r_2,r_3,r_4$\} and \{$r_{17}, r_{18}$\}. Then the EM tool classifies $r_{17}, r_{18}$ into the clusters of $r_{19}$ and $r_{20}$. Then the clusters  \{$r_1,r_2,r_3,r_4$\} and  \{$r_{15}, r_{16}, r_{17}, r_{18}$\} are correct. Next in the second round, we select an EM question $Q_M$ for asking whether $r_5$ and $r_6$ refer to the same entity.  Then the EM tool merges $r_5, r_8$ and $r_6,r_7$ and gets a correct cluster. In the third round, we ask a data repairing question \texttt{California$\leadsto$ CA}, and the machine algorithm merges $r_9, r_{10}$ and $r_{11},r_{12}$ and gets a correct cluster and correct golden value.


\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]\vspace{-1em}
\begin{center}
\centering
\includegraphics[width=0.5\textwidth]{figs/rex.eps}
\vspace{-1.5em}
\caption{Running Example for Question Scheduling\label{fig:rex}}
\end{center}
\vspace{-1.5em}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
\fi

%\lgl{add an example}
%the records do not refer to the same entity, the human requires to spilt the cluster into $c_1,c_2,\cdots, c_y$ clusters.   Then the pairs in the same cluster can be taken as matching pairs and the pairs from different clusters can be taken as non-matching pairs, and these results are taken as the training data. Here $|\qc|$ is the number of records in the cluster.


\begin{abstract}
Duplicates are prevalent in many applications, especially when integrating data from multiple sources.  Ensuring duplicate-free data analytics requires detecting these duplicates (\aka entity matching) and integrating them (\aka entity consolidation). The traditional wisdom is to treat these two steps as consecutive, \ie entity matching (EM) to find clusters of duplicates, and then entity consolidation (EC) to integrate the duplicates within the clusters which would then produce a ``golden record'', or a canonical representation, for each cluster.  However, this approach neglects two observations: (i)~EC can help EM since it can normalize or repair the data,
and (ii)~EM will get better clusters on the normalized data. 

In this paper, we propose a human-in-the-loop data integration framework that interleaves EM  and EC to maximize the golden-record accuracy. As both EM and EC need heavy human involvement, we propose a question scheduling model that judiciously selects the questions to ask.  We also consider question correlation to further improve the quality of the golden records.  Experimental results on three real-world datasets show that our holistic method can significantly improve the accuracy of golden records, compared with traditional sequential approaches. 
\end{abstract}

%Obviously, these duplicates need to be detected (\aka entity matching) and integrated (\aka entity consolidation), in order to ensure the quality of data analytics with duplicate-free data. 




